Deep-Ensemble-Based Uncertainty Quantification in Spatiotemporal Graph Neural Networks for Traffic Forecasting

Deep-learning-based data-driven forecasting methods have produced impressive results for traffic forecasting. A major limitation of these methods, however, is that they provide forecasts without estimates of uncertainty, which are critical for real-time deployments. We focus on a diffusion convolutional recurrent neural network (DCRNN), a state-of-the-art method for short-term traffic forecasting. We develop a scalable deep ensemble approach to quantify uncertainties for DCRNN. Our approach uses a scalable Bayesian optimization method to perform hyperparameter optimization, selects a set of high-performing configurations, fits a generative model to capture the joint distributions of the hyperparameter configurations, and trains an ensemble of models by sampling a new set of hyperparameter configurations from the generative model. We demonstrate the efficacy of the proposed methods by comparing them with other uncertainty estimation techniques. We show that our generic and scalable approach outperforms the current state-of-the-art Bayesian and a number of other commonly used frequentist techniques.

==> UQ_DCRNN_ arxiv/2.intro.tex <==

%\PB{first talk about about ML for traffic forecasting. Then say why Why UQ is required; do not talk about DCRNN here}. 


Traffic forecasting is a foundational component of an intelligent transportation
system. Precise forecasting across normal and extreme traffic conditions is crucial to improving traffic control, mitigating congestion, and resolving other traffic-related issues. Recently, data-driven deep learning approaches \cite{yu2017spatio, li2017diffusion, zheng2019gman} have received increased attention in traffic forecasting because of their impressive accuracy. 
However, uncertainty quantification (UQ) for traffic forecasting has received limited attention from the research community.  UQ is essential for understanding the limitations of the predictive models and how to use the models in an active traffic management system. 

Uncertainty in traffic forecasting can be decomposed into two categories: aleatoric uncertainty, which is irreducible uncertainty in the data, and epistemic uncertainty, which is uncertainty in the model \cite{tagasovska2018single}.  Aleatoric uncertainty occurs because of the inherent variability in traffic data. For example, at a given time of day, the flow and speed vary greatly. Or, faulty sensors may cause aleatoric uncertainty. This form of uncertainty is a data property, not a predictive model attribute. With aleatoric uncertainty, gathering more data in the same manner or employing a better model cannot reduce it. In contrast, regions that are underrepresented in the training dataset (out-of-distribution generalization \cite{lakshminarayanan2016simple}) can cause a mismatch between model estimation and data distribution. This situation creates epistemic uncertainty. In this case, epistemic uncertainty may be reduced by collecting more data.
%\PB{what does this mean?} \TM{explain the the term discrepancy first}
%On the other hand, uncertainty associated with the estimation of predictive model parameters or the discrepancy \PB{what does this mean?} between the model and data distribution gives rise to epistemic uncertainty in the prediction. Inadequate knowledge about the data creates a discrepancy between the model estimation and data distribution. 
% Having a lack of experience in these underrepresented regions increases the predictive uncertainty of the model. Therefore,   
Proper estimation of both the aleatoric and epistemic uncertainty for traffic forecasting is critical for understanding the limitations of the model. Furthermore, determining these uncertainty measures can be useful for detecting sensor locations where the data is most uncertain and taking measures to improve the data collection. %\PB{?? what is doubtful?} \TM{addressed}

%\PB{Introduce DCRNN here}
For decades, traffic forecasting techniques have been extensively investigated using integrated autoregressive moving average \cite{williams2003modeling}, Kalman filters \cite{kumar2017traffic}, support vector machines \cite{castro2009online, ahn2016highway}, and artificial neural networks \cite{chan2012neural,karlaftis2011statistical}. Recently, deep learning techniques have received attention because of the impressive forecasting accuracy compared with statistical approaches and traditional machine learning approaches. Researchers have explored recurrent neural networks (RNNs) and long short-term memory  networks \cite{ma2015long} and convolutional neural networks  \cite{zhang2016dnn, zhang2017deep} 
for short-term traffic forecasting. Recently, graph neural networks such as spatiotemporal graph convolutional networks \cite{yu2017spatio}, diffusion convolutional recurrent neural networks (DCRNN) \cite{li2017diffusion}, and graph multi-attention networks \cite{zheng2019gman} have achieved state-of-the-art performance by capturing the spatiotemporal dynamics of the road network. 
However, without proper quantification of the uncertainty, forecast accuracy is not trustworthy for using the model in practice. 
%\PB{for DCRNN? How abut the recent paper from Rose?}. 
%Wu et al.~\cite{wu2021quantifying}  attempted to estimate the uncertainty of graph neural networks, specifically DCRNN, by evaluating various UQ methods from both the Bayesian and the frequentist point of view. However, they did not focus on separating the aleatoric and epistemic uncertainty.

By estimating the aleatoric and epistemic uncertainty separately for traffic forecasting models, insight into whether the predictive uncertainty comes from the model or is inherently present in the data can provide insight into how to best use the model.
%If the aleatoric uncertainty is high, then collecting more data is not going to be helpful because it is the irreducible uncertainty of data. 
For example,  the 90\% quantile or 10\% quantile of the aleatoric uncertainty measure provide will predictions for the worst and best traffic conditions in a given location. 
This information can then be used to inform rerouting algorithms and other proactive traffic management strategies. 
%Instead, reducing the forecasting horizon can decrease the uncertainty in that location with high variability. 
On the other hand, if for example, the structure of the road network changes, the distribution of the training and test data may no longer represent the associated changes in the traffic patterns. This will increase the model’s epistemic uncertainty and capture the model’s lack of confidence in the forecasting results (out-of-distribution generalization \cite{lakshminarayanan2016simple}). In the absence of additional data for training, the epistemic uncertainty can be used to establish trustworthiness and to know when and where the model predictions are reliable.  

%If the epistemic uncertainty or the model uncertainty is high, then it can be reduced by collecting more training data or fine-tuning the model hyperparameters. Therefore, the separate estimation of the uncertainty from predictive models helps planners  determine how to use the uncertainty measure in practice. 
%\PB{probably you can say out of distribution detection as well? training and test data becomes different over time because of change in traffic patterns indicating model training}. \TM{Added}
%Hence, the uncertainty quantification for traffic forecasting is receiving attention recently.
%Different strategies can be built to mitigate the different sources of uncertainty.
% Write why it is important to separate two uncertainty
%\PB{We are also doing the same!} A comprehensive study for quantifying the two types of uncertainties is currently lacking in the traffic forecasting literature. \PB{need to revise}
%\PB{keep the order: aleatoric and epistemic: keep the same order }

We focus on DCRNN \cite{li2017diffusion}, one of the most promising approaches to traffic forecasting. % \PB{are you sure? can you provide evidence?}. 
It has achieved state-of-the-art performance by capturing both spatial and temporal dependencies of the traffic network through a combination of graph and recurrent neural networks. Our proposed approach for uncertainty estimation in DCRNN is comprised of the following steps:
\begin{itemize}
    \item The DCRNN is configured to model the distribution of traffic data using simultaneous quantile regression (SQR).
    \item A scalable Bayesian optimization method is used to tune the hyperparameters of the DCRNN model with simultaneous quantile regression.
    \item A set of high-performing hyperparameter configurations from the hyperparameter optimization is used to fit a generative model; this captures the joint probability distribution of the high-performing hyperparameter values. A new set of hyperparameter configurations is then sampled from the generative model, and the corresponding DCRNN model are trained simultaneously.
    \item A set of high performing models is selected for ensemble construction and a variance decomposition approach is then used to estimate the aleatoric and epistemic uncertainties from the ensemble predictions.   
\end{itemize}
The main contributions of the paper are:
\begin{itemize}
    \item A scalable approach to construct deep ensembles using Bayesian hyperparameter optimization and generative modeling,  
    \item A conceptually simple, yet effective, Gaussian assumption-free uncertainty quantification approach to quantify uncertainty of a DCRNN model,
    \item The first demonstration of aleatoric and epistemic uncertainty estimation for short-term traffic forecasting, and
    \item A demonstrated improvement over the state-of-the-art Bayesian DCRNN trained by stochastic gradient Markov Chain Monte Carlo for uncertainty estimation in DCRNN.
\end{itemize}

%Our approach outperforms the state-of-the-art Bayesian neural network method and a variety of other frequentist uncertainty techniques.
%We quantify the aleatoric uncertainty in DCRNN using the simultaneous quantile regression (SQR) \cite{tagasovska2018single} method and epistemic uncertainty using the deep ensemble method \cite{lakshminarayanan2016simple}. SQR \cite{tagasovska2018single} adopts a \PB{pin ball?} loss function to learn all quantiles in a single model. \PB{you have to say what the method is?}. This method is simple, scalable, easy to implement, and not explored for traffic forecasting. Similarly, we develop a deep ensemble method for epistemic uncertainty quantification as the previous studies \cite{lakshminarayanan2016simple, liu2019accurate} show that ensembles  boost the predictive performance of the model compare to single model \PB{not clear! what do you mean?}\TM{Added} \PB{not clear review; introduce the approach}. \PB{these methods are already proposed; what is the novelty?} Moreover, this method can be parallelized easily and it has not been explored for traffic forecasting earlier. \PB{have to revise!}

\begin{comment}
Here we summarize our contributions of this paper:
\PB{these are not contributions}
\begin{itemize}
    \item Estimate the aleatoric and epistemic uncertainty for each sensor location using DCRNN
    \item Compare the deep ensemble and SQR method with the other UQ estimation techniques 
    \item Compute the traffic dynamics of each sensor location and relate the estimated uncertainty with the traffic dynamics
    \item Validate the aleatoric uncertainty with ground truth data
\end{itemize}
\end{comment}




==> UQ_DCRNN_ arxiv/3.related.tex <==
% \begin{itemize}
%     \item Uncertainty estimation for traffic forecasting 
%     \item Spatio-temporal forecasting using Graph neural network
%     \item Uncertainty quantification for spatio-temporal forecasting
%     \begin{itemize}
%         \item Epistemic uncertainty
%         \item Aleatoric uncertainty
%     \end{itemize}
% \end{itemize}


%Traffic forecasting provide critical input to the traffic management system. Lately, data driven deep learning methods achieved notable performance on traffic forecasting. Despite of the highly accurate forecasting results, there is high level of uncertainty in long-term traffic forecasting. Quantifying the uncertainty estimation is critical to provide a trustworthy solution.
%Whereas, other data driven methods either capture spatial or temporal dependencies such as ...
%\PB{this is a repeat of what is said before in the intro}
%Uncertainty quantification is receiving attention for traffic forecasting. 

%\PB{I reduced the redundancy by moving the text from intro to the related work; revise this section and make it coherent.}
Quantifying predictive uncertainty is important for deep learning models. 
Various methods for quantifying uncertainty, such as \cite{abdar2021review, hullermeier2021aleatoric}, have been investigated over the past decade.  In this paper  we look at the uncertainty quantification techniques that are used specifically in traffic forecasting.

Uncertainty quantification has not yet been  extensively adopted for traffic forecasting.
Only a few attempts have been made to measure uncertainty in highway traffic forecasts.
The generalized autoregressive conditional heteroscedasticity (GARCH) \cite{guo2010real, guo2014adaptive, tsekeris2010short} model was used to estimate the uncertainty of traffic forecasting with a Kalman filter.  A bootstrapping technique ass used by Matas et al. \cite{matas2012traffic} for uncertainty estimation. Quantile regression recently has been  developed to forecast traffic volumes with confidence intervals \cite{hoque2021estimating}. Bayesian neural networks were used \cite{van2009bayesian, mazloumi2011prediction, zhu2017deep} to predict the travel time along with the confidence intervals.  All of these methods, however, perform forecasting on individual locations. None of the  methods consider spatiotemporal dynamics of all the locations together in their models.

Recently, Wu et al.~\cite{wu2021quantifying} developed and tested six uncertainty estimation techniques for DCRNN. These include five frequentist methods---bootstrap,  MIS,  quantile regression, spline quantile regression,  Monte Carlo  dropout, and one Bayesian model trained through 
%Stochastic Gradient Markov chain Monte Carlo (
SG-MCMC. 
They compared these strategies empirically and reported on the effectiveness and computational trade-offs of various UQ methods. According to their experimental results, Bayesian DCRNN with SG-MCMC results in superior mean prediction when compared to the five frequentist methods but it is computationally expensive. Frequentist approaches, on the other hand, are inexpensive and effective in covering data variations. The uncertainty calculated in Bayesian DCRNN is the total uncertainty, a combination of both epistemic and aleatoric; it cannot distinguish between the two types of uncertainty. Moreover, Bayesian neural networks are computationally more expensive to train than their deterministic counter parts and typically do not scale well for large data sets due to the sequential nature of the specialized training procedures.

Our method is robust in mean predictions and is effective in covering variations in the data. Moreover, the hyperparameter estimation and ensemble can be scaled over multiple compute nodes. Overall, our method is more effective and more efficient compared with other Bayesian and frequentist approaches in terms of accuracy and scalability.

Our approach was inspired by four recent works on uncertainty estimation through deep ensembles: deep ensemble~\cite{lakshminarayanan2017simple}, hyper ensemble~\cite{wenzel2020hyperparameter}, neural ensemble search \cite{zaidi2021neural}, and joint neural and hyperparameter search ensembles \cite{egele2021autodeuq}. 
These methods assume a Gaussian distribution for the output variable, perform regression on a single variable, do not make use of scale for hyperparameter search to generate ensembles, and do not adopt generative modeling. The uniqueness of our method stems from 1) its application to spatial temporal graph neural networks, 2) inclusion of Gaussian-assumption-free simultaneous quantile regression, 3) multi-output spatial temporal regression, 4) the use of hyperparameter search at scale, and 5) Gaussian copula generative modeling for ensemble construction.


%\PB{what was the outcome?}

%Uncertainly estimation for spatiotemporal forecasting specifically DCRNN is not explored widely. 


%Distinguishing two source of uncertainty is important to understand whether the uncertainty is coming from the data (aleatoric) or from the model (epistemic). The data or the aleatoric uncertainty is irreducible whereas the epistemic uncertainty can be reduced by tweaking the model or adding more data. Proper quantification of distinct source of uncertainty could be useful for uncertainty informed decision making.    


% \subsection{Aleatoric uncertainty}
% Aleatoric uncertainty is captured by learning the conditional distribution of target variable given the input variable. There are very few studies, which estimate the aleatoric uncertainty for the traffic forecasting. In general, one common approach is to assume that the conditional distribution is Gaussian \cite{kendall2017uncertainties, rasmussen2003gaussian}. This approach is redistricted to estimate the Gaussian aleatoric uncertainty. Another approach use generative models  \cite{mohamed2016learning} such as conditional generative adversarial networks \cite{mirza2014conditional} and DiscoNets \cite{bouchacourt2016disco}. However, these models are difficult to train and experience 'mode collapse' problem \cite{goodfellow2016nips}. Another popular approach is performing quantile regression \cite{takeuchi2006nonparametric, zheng2010boosting}. This method is also used in the traffic domain \cite{hoque2021estimating} to estimate the uncertainty of future forecasts. However, these methods perform regression on a fixed quantile level. Whereas, simultaneous quantile regression \cite{tagasovska2018single} that we leverage estimates all the quantiles jointly and effectively capture non-Gaussian, asymmetric, skewed, and heteroskedastic noise of the data in single model. 

% %Moreover, this technique has not been used to estimate the aleatoric uncertainty for traffic forecasting.

% \subsection{Epistemic uncertainty using ensemble learning}
% A regularly used technique to approximately measuring the epistemic uncertainty is to use an ensemble of neural network models \cite{abdar2021review, liu2019accurate}. Using this technique multiple models are trained and they produce multiple predictions and empirical variance of model prediction gives an approximate measure of the epistemic uncertainty.
% Lakshminarayanan et al. \cite{lakshminarayanan2016simple} shows that simple non-Bayesian deep ensemble learning can provide robust uncertainty quantification compare to Bayesian techniques. Ensemble learning is used in different domains for time series forecasting such as water quality forecasting \cite{shamshirband2019ensemble}, clinical time series for healthcare related tasks \cite{wickstrom2020uncertainty}, wind  power prediction  \cite{giebel2007ensemble}. Ensemble technique has not been used for measuring uncertainty for spatiotemporal traffic forecasting. 


% Hullermeier et al. \cite{hullermeier2021aleatoric} shows the importance of distinguishing two different source of uncertainty for supervised learning \PB{for traffic?}. Nguyen \cite{nguyen2019epistemic} separate the two source of uncertainty in active learning set-up and found that epistemic uncertainty is more appropriate than aleatoric as a selection criteria. Senge et al.\cite{senge2014reliable} shows the importance of separately estimating two source of uncertainty in medical decision making. \PB{so none of these were done in the context of traffic forecasting; if so you have to move this after traffic forecasting UQ} Next, we survey the relevant work for estimating the aleatoric and epistemic uncertainty for traffic forecasting. 


% \PB{I am confused about the structure of the related work; What are you trying to achieve with the related work. You have to establish the novelty of the proposed methods in the paper not just survey the related work}

%\PB{move the related work on UQ }

%Our approach addresses two sources of uncertainty --  aleatoric and epistemic for DCRNN using SQR and deep ensemble. To the best of our knowledge, this is the first work to investigate the usefulness of predictive uncertainty by correlating the uncertainty with sensor level traffic dynamic for real word deployment of forecasting model.



==> UQ_DCRNN_ arxiv/4.0.dcrnn.tex <==
The DCRNN considers the road network as a weighted directed graph $G = (V, E, A)$, where the set $V$ of nodes represents $N$ traffic measurement (sensor) locations, the set $E$ of edges represents the connectivity between the nodes,
and the adjacency matrix  $A$ ($A \in R^{N\times N}$) represents the proximity between the nodes. 
Given the graph $G$ and historical time series data of traffic metrics $X$,  DCRNN seeks to learn a function \text{f(.)} to forecast short-term traffic metrics for $K$ time steps given the past $K'$ traffic metrics as input:
\begin{equation*}
X(k-K'+1), ...,X(k); G \xrightarrow{\text{f(.)}} X(k+1),... , X(k+K),
\end{equation*}
where $X(k) \in \mathcal{R}^{N \times 1}$ is a vector of traffic metrics defined over $N$ vertices at time step $k$. %\PB{What is $G$ doing here?}

%Given the past traffic metrics for $K'$ timestamps $X(t-K'+1)$ to $X(t)$, the goal is to forecast the traffic metrics for $K$ timestamps $X(k+1)$ to $X(k+K)$. To denote future time series, we use the notation $y\in Y$. Our data has $N$ sensor locations and for each locations we have $n$ timestamps $\{x_i, y_i\}_{i=1}^n$, where $ x\in X$ and $y \in Y$ are the historical and future traffic metrics. $\hat{y}$ represents the forecasted timeseries, where $X\in \mathcal{R}^{N*K'}$,  $Y\in \mathcal{R}^{N*K}$,  $x\in \mathcal{R}^{1*K'}$, and $y\in \mathcal{R}^{1*K}$   %\TM{added here} 


 DCRNN is an encoder-decoder neural network architecture with RNN layers that operates on a graph. It models the temporal dependency of the traffic using gated recurrent units (GRUs), a variant of RNN. Specifically, the matrix multiplications of the GRU cell are replaced by a diffusion-convolutional operation
%The diffusion convolution operation is used inside each GRU cell 
to model the spatial dependency of the road network. The modified GRU cell is defined as
\begin{equation}\label{equ_1}
\begin{array}{lcl}
r^k & = &  \sigma (W_{r\bigstar G} [X(k), h_{k-1}] + b_r) \\
u^k & = &  \sigma (W_{u\bigstar G} [X(k), h_{k-1}] + b_u) \\
c^k & = &  \tanh (W_{c\bigstar G} [X(k) (r_k \odot h_{k-1}] + b_c) \\
h_k & = & u_k \odot h_{k-1} + (1 - u_k) \odot c_k ,
\end{array}
\end{equation}
where $X(k)$ and $h_k$ represent the traffic state and final state
at time $k$, respectively;
%GAIL - is X(t) the same as X(k) -- I don't see X(t) in the above equation
$u_k$, $r_k$, and $c_k$ are the update gate, reset gate, and cell state, respectively; $\bigstar G$ denotes the diffusion-convolution operation; and $W_r, W_u,$ and $W_c$ are parameters of the GRU cell.
The diffusion-convolution operation $\bigstar G$ on the graph $G$ is defined as
\begin{equation}
\label{equ_2}
 W_{(\cdot)\bigstar G} X = \sum_{d=0}^{\mathcal{K}-1} (W_{(\cdot)O} (D_O^{-1}A)^d + W_{(\cdot){I}}(D_I^{-1}A)^d) X,
\end{equation}
where $\mathcal{K}$ is a maximum diffusion step;  $D_O$ and $D_I$ are the in-degree and out-degree diagonal matrices, respectively; $A$ is the adjacency matrix; and $W_O$ and $W_I$ are the learnable filters for the diffusion process and reverse one, respectively.
%\PB{where was these things defined!}.

The encoder takes the input adjacency matrix and $K'$ time series data and maps the data into a latent representation. The decoder takes the latent representation and produces forecasts for future traffic for $K$ timestamps. In the training,  DCRNN optimizes the following mean absolute error (MAE) loss using a minibatch stochastic gradient algorithm:
\begin{align}
 \hat{f} \in \operatorname*{argmin}_{f}   \frac{1}{N} \mathlarger{\mathlarger{\sum}}_{j=1}^{N} \frac{1}{n} \mathlarger{\mathlarger{\sum}}_{i=1}^{n} | y_{ij} - \hat{y}_{ij}|, 
\label{mae}
\end{align}
% \text{loss\textsubscript{MAE}} &=  \frac{1}{n}\sum_{i=1}^n | y_i - \hat{y}_i |
%\end{equation*}
%\end{linenomath}
where $y$ and $\hat{y}$ are, respectively, the observed and corresponding forecast values for the $i^{th}$ time step and $j^{th}$ sensor location;  $n$ is the total timestamps for each sensor locations; and $N$ is the total number of sensor locations. 



==> UQ_DCRNN_ arxiv/4.method.tex <==
%\subsection{Diffusion Convolutional Recurrent Neural Network (DCRNN)}
%For spatiotemporal forecasting using DCRNN, 

%Given the past traffic metrics for $K'$ timestamps $X(t-K'+1)$ to $X(t)$, the goal is to forecast the traffic metrics for $K$ timestamps $X(k+1)$ to $X(k+K)$. To denote future time series, we use the notation $y\in Y$. Our data has $N$ sensor locations and for each locations we have $n$ timestamps $\{x_i, y_i\}_{i=1}^n$, where $ x\in X$ and $y \in Y$ are the historical and future traffic metrics. $\hat{y}$ represents the forecasted timeseries, where $X\in \mathcal{R}^{N*K'}$,  $Y\in \mathcal{R}^{N*K}$,  $x\in \mathcal{R}^{1*K'}$, and $y\in \mathcal{R}^{1*K}$   %\TM{added here} 

We focus on uncertainty quantification in DCRNN predictions. Our proposed method, DCRNN with simultaneous quantile regression (DCRNN-SQRUQ),
seeks to  estimate both aleatoric (data) and epistemic (model) uncertainties. Our methodology has four steps, as illustrated in  Figure \ref{fig_diagram}: (1) simultaneous quantile regression (SQR) loss for  DCRNN, (2)  hyperparameter optimization using scalable Bayesian optimization method, (3) high-performing hyperparameter generation using a Gaussian copula model, and (4) aleatoric and epistemic uncertainty estimation using variance decomposition for deep ensemble. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/dia.png}  
\caption{Components of our proposed approach DCRNN-SQRUQ: (1) simultaneous quantile regression (SQR) loss for DCRNN, (2) Bayesian hyperparameter optimization, (3)  high-performing hyperparameter generation using a Gaussian copula method, and (4) uncertainty estimation using variance decomposition for deep ensemble.}
\label{fig_diagram}
\end{figure}

\subsection{Simultaneous quantile regression} \label{sqr}
The first step of our approach is the adaptation of SQR in  DCRNN to predict the quantiles of the forecasting traffic distribution.

Consider a typical regression setting consisting of input features $X$ and output variable $Y$ taking real values $y$. Let $F(y)=P(Y \leq y)$ be the cumulative distribution function of $Y$; the $q^{th}$ quantile of $Y$ can be calculated by the quantile distribution function $F^{-1}(q) = inf (y:F(y) \geq q)$, where $q \in (0, 1)$. The quantile regression approach seeks to model $\hat{y}=\hat{f}_{q}(x)$ that approximates the conditional quantile distribution function $y=F^{-1}(q \mid X=x)$. Specifically, the quantile regression estimates the value of $Y$ at a given quantile $q$ conditioned on the given $x$ values of input features $X$. This estimation can be achieved by using  the pinball loss function \cite{fox1964admissibility, koenker1978regression}:
\begin{equation}
\ell_{q}(y, \hat{y})=\left\{\begin{array}{lr}
q(y-\hat{y}) & \text { if } y-\hat{y} \geq 0 \\
(1-q)(\hat{y}-y) & \text { else }
\end{array}\right.
\end{equation}
Building on this, the recently proposed SQR approach estimates all the quantiles simultaneously by solving the following optimization problem:  
\begin{equation}
\hat{f} \in \arg \min \frac{1}{n} \sum_{i=1}^{n} \underset{q \sim U[0,1]}{\mathbb{E}}\left[\ell_{q}\left(f\left(x_{i}, q\right), y_{i}\right)\right] .
\label{sqr}
\end{equation}
This optimization problem is solved by using minibatch stochastic gradient descent, where random quantile levels $q \sim U[0,1]$ (uniform distribution) are sampled afresh for each training point and for each minibatch. 

In DCRNN, for each sensor location and for each forecast time step, we seek to estimate the traffic metric at all quantiles conditioned on the past $K'$ traffic metrics defined over $N$ sensor locations. This is achieved by replacing the MAE loss minimization with the SQR minimization. Applying Eq.~\ref{sqr} in Eq.~\ref{mae}, we get
\begin{equation}
    \hat{f} \in \operatorname*{argmin}_{f} \frac{1}{N} \mathlarger{\mathlarger{\sum}}_{j=1}^{N} \frac{1}{n} \mathlarger{\mathlarger{\sum}}_{i=1}^{n} \operatorname*{\mathbb{E}}_{q \sim U[0, 1]} [l_{q} (f(x_{ij}, q,G),y_{ij})].
\end{equation}

\begin{comment}
%To that end, instead of using MAE as the DCRNN loss, we use Simultaneous Quantile Regression Loss to model the distribution of $Y$ given the input $X$ and the graph $G$. 
%The regression problem of traffic forecasting can expressed similarly, where the input $ x_i\in X$ and the output $y_i \in Y$ are the traffic metrics for $K'$ is past time steps and $K$ is the future time steps. Let $\hat{y}$ represents the forecasted timeseries, and $X\in \mathcal{R}^{N*K'}$, and  $Y\in \mathcal{R}^{N*K}$, where, for each of the $N$ locations we have $n$ timestamps $\{x_i, y_i\}_{i=1}^n$.
%Given the input timeseries $X$, and the graph $G$, DCRNN estimate the target timeseries $Y$. 
%Instead of minimizing the MAE, we modify the DCRNN loss to model the distribution of $Y$ given the input $X$ and the graph $G$. 
%We estimate the quantile level ($\tau$) of the target variable $Y$ 
%When the mean traffic condition is insufficient to make a judgment, different quantiles ($\tau$) of the target variable will assist us determine the worst and best case traffic conditions of a roadway by looking at the 90 percent quantile or 10 percent quantile.
%Let $Y$ be a real valued random variable with cumulative distribution function $F(y) = P (Y < y)$ takes real values $y$.  The $\tau^{th}$ quantile of Y can be calculated by $F^{-1}(\tau) = inf (y:F(y) \geq \tau)$, where $\tau\in (0, 1)$. The aim of the quantile regression is to estimate a given quantile $\tau$ of the target $Y$ given $X$. 
% \PB{ explain pin ball loss with a figure if possible} %\\PB{you have to introduce quantiles; }TM{introduced quantile in the paragraph above}
The DCRNN model forecast for traffic $\hat{y}$ given the input $x$ and the graph $G$ for a single quantile level can expressed as $\hat{y} = f_{q}(x, G)$ %\PB{this is confusing; does not follow the notations introduced before} %\TM{introduced the symbols}.
The pinball loss function for DCRNN can be written as

\begin{equation*}
l_{q}(y_i, f(x_i, G)) = 
    \begin{cases}
      q (y_i - f(x_i, G)) & \text{if} (y_i - f(x_i, G)) \ge 0, \\
      (1-q) (f(x_i, G) - y_i) & \text{else} ,\\
    \end{cases}   
\end{equation*}

% \begin{equation*}
% \begin{array}{cc}
%       l_{\tau} (y, \hat{y}) = &  \tau (y - \hat{y}), \text{ if } y \ge \hat{y}   \\
%                               & (1 - \tau) (\hat{y} - y), \text{ if } \hat{y} > y,
% \end{array}
% \end{equation*}
where $y_i$  is the observed value of target variable $Y$,  $x_i$ is the input value, and $G$ is the input graph. 
%\PB{this was already used in the previous paragraph as future traffic} \TM{changed it the previous paragraph} are the observed and forecasted value of target variable $Y$.
%The input and target pairs ($x_1$, $y_1$), ... ($x_n$, $y_n$) on each node of the graph come from some unknown probability distribution P(X,Y) %\PB{not clear; also the $x$, $y$ business; you have to introduce them properly; it is all confusing!}\TM{now introduced in DCRNN section} 
%and there are $N$ such nodes in the graph. 
The quantile distribution of Y given X and G at a single quantile level can be estimated by solving:
\begin{equation*}
    \hat{f}_{q} \in \operatorname*{argmin}_{f} \frac{1}{N} \mathlarger{\mathlarger{\sum}}_{j=1}^{N} \frac{1}{n} \mathlarger{\mathlarger{\sum}}_{i=1}^{n} l_{q} (y_{ij}, f(x_{ij}, G)),
\end{equation*}
%\PB{in the previous equation, the first argument for $l_r$ is observed value; here it is predicted; notations are a big mess!} \TM{rectified}
%where, $N$ is the total number of nodes in the graph and $n$ is the all timestamps for single location. 
Instead of solving the problem for a single quantile, it is possible to  estimates all quantile levels simultaneously using simultaneous quantile regression (SQR) by solving:

\begin{equation*}
    \hat{f} \in \operatorname*{argmin}_{f} \frac{1}{N} \mathlarger{\mathlarger{\sum}}_{j=1}^{N} \frac{1}{n} \mathlarger{\mathlarger{\sum}}_{i=1}^{n} \operatorname*{\mathbb{E}}_{q \sim \mathcal{U} [0, 1]} l_{q} (y_{ij}, f(x_{ij}, q,G))
\end{equation*}
%\PB{Why $\hat{f}$ in this Eq?} \TM{didn't understand the question}
SQR sample the quantile levels randomly ($q \sim \mathcal{U}$[0, 1]) for each mini-batch and minimize the loss using Adam optimizer during DCRNN training. This method can be assumed as the randomized version of the pin ball loss function. %As result of minimizing multiple quantiles simultaneously, the this method become capable to compute any quantile of the target variable Y given X. Finally,


% Variance of the conditional distribution of the target given the input is basically the aleatoric uncertainty. Hence, optimizing quantiles helps to get the conditional distribution of the target or aleatoric uncertainty by estimating in the (1 - $\rho/2$) and $\rho/2 $ quantile around the median for (1 - $\rho$) confidence interval.

% \begin{equation*}
% U_a = f(x, 1 - \rho/2, G) - f(x, \rho/2, G)
% \end{equation*}

%\PB{overall, why optimizing quantiles help you to capture ale uncertainty?} %\TM{wrote}
\end{comment}

The key advantages of SQR include well-calibrated prediction intervals; joint estimation of the quantiles that can eliminate the unacceptable crossing quantiles \cite{takeuchi2006nonparametric}; and the ability to model non-Gaussian, skewed, asymmetric, multimodal, and heteroskedastic noise in the data. 

 
%Our dataset consist of $N$ sensor locations and for each locations we have $n$ timestamps $\{x_i, y_i\}_{i=1}^n$, where $ x\in X$ and $y \in Y$ are the historical and future traffic metrics \PB{this should come way before; just below the first eq in III.A }. 
%We estimate the epistemic uncertainty of DCRNN model using deep ensemble method. Using this deep ensemble method, we compute the probabilistic distribution of the output $p_{w} (Y|X, G)$ given the input timeseries $X$ and graph $G$, where $W$ are the parameters of the DCRNN network \PB{this is essentially ale uncertainty}. 
 %\PB{wrong! $W_1, ..., W_m$ are trained parameters as per your definition in the previous paragraph} \TM{those are the parameters of DCRNN...start with random initialization} and train the model on the entire training dataset. MAE loss is minimized for each network \PB{Why you did not use SQR?}. 

% To model aleatoric uncertainty, we use the quantiles from SQR. our estimate of aleatoric uncertainty is (1 - $\rho/2$) and $\rho/2 $ quantile around the median for (1 - $\rho$) confidence interval. We construct $M$ models for deep ensemble. Therefore, the 
% \begin{equation*}
% U_a = \frac{1}{M}\sum_{i = 0}^{M} f(x, 1 - \rho/2, G) - f(x, \rho/2, G)
% \end{equation*}

% To model epistemic uncertainty, deep ensembles \cite{lakshminarayanan2016simple} is used. The ensemble is treated as a mixture of uniformly-weighted models, and the predictions are combined as follows:

% \begin{equation*}
%     p(Y|X, G) = M^{-1} \sum_{m=1}^M P_{W_m}(Y|X, W_m)
% \end{equation*}

% To estimate the final prediction from the ensemble predictions, we consider all the networks and treat their results as a mixture of Gaussian distributions. Finally, compute the mean and variance of Gaussian distributions as:

% \begin{equation*}
%     \mu_*(x) = \frac{1}{M} \sum_{i=1}^M \mu_{W_i} (x)
% \end{equation*}

% \begin{equation*}
%   U_e = \sigma_*(x) = \sqrt{ \sum_{i=1}^M \frac{\mu_{W_i} (x) - \mu_* (x)}{M}}
% \end{equation*}



%\begin{equation*}
%    \sigma_*^2(x) = \frac{1}{M} \sum_{i=1}^M \mu^2_{W_i} (x) - \mu_*^2 (x)
%\end{equation*}

%Here, the variance is the epistemic uncertainty. This estimation goes low if all mean estimations are similar and high if the mean estimates diverge extensively. The variance reflects the spread of prediction among multiple models while neutralising the noise of data. Thus ensemble captures the  epistemic uncertainty.


\subsection{Scalable hyperparameter optimization}

The second step of our approach is the use of a scalable hyperparameter search for tuning the hyperparameters of DCRNN. 

DCRNN has several training hyperparameters, including  batch size, a threshold \texttt{max\_grad\_norm} to clip the gradient norm to avoid exploring gradient problem of RNN \cite{pascanu2013difficulty}, initial learning rate and learning rate decay, maximum diffusion steps, and architecture
configurations (network topology parameters) such as number of encoder and decoder layers,  number of RNN units per layers, and filter type (i.e., random walk, Laplacian). The hyperparameters are crucial in determining  DCRNN's forecasting accuracy.

%Given the real dataset, we aim to maximize model performance. Therefore, 

To tune the hyperparameters of the DCRNN model with SQR, we use the DeepHyper  \cite{balaprakash2018deephyper} open source software that has a scalable Bayesian optimization (BO) method.  Given the training and validation data, a neural network model, and the feasible set of values of the training hyperparameters, DeepHyper uses an asynchronous BO method seeks to minimize the validation error by repeatedly training the neural network model with various hyperparameter values. The DeepHyper BO uses an incrementally updated random forest model to learn the relationship between the hyperparameter values and their corresponding validation errors. The BO method uses the random forest model to predict the validation errors of the evaluated hyperparameter configurations along with the uncertainty associated with the predicted value. The BO search  involves both evaluation of hyperparameter configurations, where the random forest model is most uncertain, and exploitation, focusing on hyperparameter configurations that are closer to the previously found high-performing configurations. The balance between  exploration and exploitation is achieved by selecting an unevaluated hyperparameter configuration $\boldsymbol{x}^{*}$ that minimizes the lower confidence bound ($\mathrm{LCB}$) acquisition function:
\begin{align}
\boldsymbol{x}^{*}=\underset{\boldsymbol{x} \in \mathcal{D}}{\arg \min } \underbrace{\hat{\mu}(\boldsymbol{x})-\lambda \times  \hat{\sigma}(\boldsymbol{x})}_{\mathrm{LCB}},
\end{align}
where $\hat{\mu}(\boldsymbol{x})$ and $\hat{\sigma}(\boldsymbol{x})$ are respectively the predicted estimate and the standard deviation of that estimate from the random forest model of the given unevaluated hyperparameter configuration $\boldsymbol{x}$ sampled from the hyperparameter space $\mathcal{D}$ and where $\lambda$ is a user-defined parameter that controls the trade-off between the exploration and exploitation. 

%\begin{align}
%\mathrm{LCB}(\boldsymbol{x}, \lambda)=\hat{\mu}(\boldsymbol{x})-\lambda \hat{\sigma}(\boldsymbol{x})
%\end{align}

A key reason for choosing DeepHyper for the DCRNN hyperparameter tuning is scalability. The DeepHyper BO follows a single-manager multiple-workers parallization scheme, where the manager runs the search,  generates hyperparameter configurations, and sends them to workers for evaluation; each worker is responsible for evaluating a hyperparameter configuration by training the neural network model with the given configuration, computing the validation error, and returning that value to the manager. The manager generates hyperparameter configurations for evaluation in an asynchronous manner: as soon as one or more workers returns the validation error, the manager uses the returned values to retrain the surrogate model within the BO and generates the next hyperparameter configuration for the worker. To enable simultaneous multiworker evaluations, the BO uses a constant liar scheme, where configurations are generated sequentially by refitting the random forest model with a lie for the validation error, given by a predicted value from the model itself, for the previously selected unevaluated hyperparameter configuration.

%generates a set of high-performing hyperparameter configurations use Asynchronous Model Based Search (AMBS) method. AMBS trim the search space towards the promising region by fitting a surrogate model to learn the link between different configurations of hyperparameters and their validation error. Because of its asynchronous nature, AMBS does not wait for all assessments to be completed. The validation error is used to narrow the search space shortly after an evaluation is completed. Deephyper builds the surrogate model using random forests, and AMBS supports continuous, discrete, or nonordinal category search space. The scalability and portability of AMBS on high-performance computing (HPC) systems are the two advantages of adopting Deephyper over other hyperparameter search methods. AMBS is based on a manager-worker paradigm, in which the manager creates the configurations and the workers assess them in parallel on separate nodes of the HPC system, returning the validation errors to the management to create new configurations.\PB{very poor writing and exposition!! You use DeepHyper/HPS day in day out but you do not know how to describe this!}

%In our approach, we generate a large number of hyperparameter configurations and select set of high-performing configurations for our next method based on the objective function of the hyperparameter optimization. 

We use DeepHyper to tune the hyperparameters of DCRNN not only to find the best hyperparameter configuration with minimal validation error but also to extract a set of hyperparameter values with minimal validation errors for generative modeling. Moreover, we scale the hyperparameter search on an increasing number of compute nodes to see how scaling impacts the overall uncertainty estimation in DCRNN. 

\subsection{Generative modeling and ensemble training}
The third step of our approach is generative modeling.  We model the joint probability distribution of the high-performing hyperparameter configurations from the previous step and use the distribution for  generating more high-performing hyperparameter configurations to train an ensemble of DCRNN models. 

%Given a set of a high-performing hyperparameter configurations, 

Copula is a statistical approach used to model the joint probability distribution of a given set of random variables by analyzing the dependencies between their marginal distributions.
We use a multivariate Gaussian copula model \cite{schmidt2007coping} to learn the joint probability distribution between high-performing hyperparameter configurations.  
%A set of high-performing hyperparameter configurations from the hyperparameter optimization is used to fit a multivariate Gaussian copula model \cite{schmidt2007coping}. 
The copula model $C$ takes multiple marginal distributions of the hyperparameters  $u_1, u_2,..., u_{hp}$ and returns a multivariate distribution as follows:
\begin{equation}
    C(u_i, u_2, ..., u_{hp}) = \Phi_{\sum} (\Phi^{-1}(u_1),  \Phi^{-1}(u_2), ..., \Phi^{-1}(u_{hp})),
\end{equation}
where $\Phi_{\sum}$  represents the cumulative distribution function (CDF) of a multivariate normal, with covariance $\sum$ and mean 0, and $\Phi^{-1}$ is the inverse CDF for the standard normal. This captures the joint probability distribution of the high-performing hyperparameter values such as learning rate, batch size, number of layers, and objective function. 

The rationale for generative modeling through multivariate Gaussian copula is twofold. First, in hyperparameter search problems characterized by integer, real, and categorical hyperparameters, there are multiple high-performing regions; while BO cannot sample these regions uniformly, it can sample a few configurations from different high-performing regions. By selecting these high-performing configurations and fitting a Gaussian copula, we can sample from the sparsely sampled high-performing regions as well. Second, if we have to find more high-performing configurations from different regions directly with BO, then we have to run the search multiple times with different initialization; this process will be both computationally expensive and resource intensive.

Once the copula model $C$ is trained, we sample a number of hyperparameter configurations from  $C$ and run multiple DCRNN training sessions with the sampled hyperparameter configurations. From these trained DCRNN models, we select a set of high-performing models for ensemble construction. 

%Top 25\%, quantile models are selected for comparison with other UQ techniques. 
%A new set of $M$ hyperparameter configurations are then sampled from distribution. Those high-performing hyperparameter configurations are used to train $M$ models simultaneously. 


\subsection{Variance decomposition for DCRNN ensembles}

The fourth step of our approach is to use the  ensemble of DCRNN models to estimate the traffic metrics and the associated aleatoric and epistemic uncertainty using variance decomposition.

%Given the input, output and the graph, we attempt to model aleatoric and epistemic uncertainty using our model DeepSQRUQ based on deep ensemble \cite{lakshminarayanan2016simple}. For the ensemble, we train $M$ is the number of DCRNN networks with SQR loss function discussed in section \ref{sqr}. 

Let  $\mathcal{E} = {\theta_{i}, i = 1, 2,..., M}$ be the ensemble of $M$ models.  Previous studies have showed that if each model is configured to predict the mean and variance of an output distribution that is assumed to be  Gaussian and if the model is trained with negative log likelihood loss \cite{egele2021autodeuq},  the empirical estimation of the mean and the total variance can be written as follows.   
\begin{equation}
\begin{split}
\mu_{\mathcal{E}}     &  = \frac{1}{M}\sum_{\theta \in \mathcal{E} } \mu_{\theta} \\
\sigma_\mathcal{E}^2  &  = \underbrace{\frac{1}{M} \sum_{\theta \in \mathcal{E}} \sigma^2_\theta}_{ \text{Aleatoric Uncertainty} } + \underbrace{\frac{1}{M-1} \sum_{\theta \in \mathcal{E}} (\mu_\theta - \mu_\mathcal{E})^2}_{ \text{Epistemic Uncertainty}}
\label{eq:var-decomposition-1}
\end{split}
\end{equation}
The total uncertainty quantified by $\sigma_\mathcal{E}^2 $ is a combination of aleatoric and  epistemic uncertainty, which is given by the mean of the predictive variance of each model in the ensemble and the predictive variance of the mean of each model in the ensemble.  

%In our method, we generate number of DCRNN models $\mathcal{E} = {\theta_{i}, i = 1, 2,..., M}$, where $\mathcal{E}$ is the set of $M$ models present in the ensemble, $\theta$'s are the models with different hyperparameters and architectural configurations and $M$ is the size of the ensemble. In the Gaussain assumption setting \cite{egele2021autodeuq},  

Our proposed SQR-based DCRNN seeks to predict quantiles of the distribution as opposed to the mean and variance of the distribution. Thus it is more generic and free from Gaussian assumptions. We derive the empirical estimate of the median ($q_{50\%}$) and the total variance of the ensemble as
\begin{align}
\begin{aligned}
{q_{50\%}}_{\mathcal{E}}     &  = \frac{1}{M}\sum_{\theta \in \mathcal{E} } {q_{50\%}}_{\theta} \\
\sigma_\mathcal{E}^2  &  = \underbrace{\frac{1}{M} \sum_{\theta \in \mathcal{E}}  (\frac{{q_{66\%}}_\theta - {q_{33\%}}_\theta}{2})^2}_{ \text{Aleatoric Uncertainty} }\\  & \qquad \qquad \qquad +\\ 
 &  \qquad \underbrace{\frac{1}{M-1} \sum_{\theta \in \mathcal{E}} ( {q_{50\%}}_\theta - {q_{50\%}}_\mathcal{E})^2}_{ \text{Epistemic Uncertainty}},
\label{eq:var-decomposition-2}
\end{aligned}
\end{align}
where $q_{33\%}$ and $q_{66\%}$ are the 33\% and 66\% quantiles of the output distribution, respectively. 

Note that Eq. \ref{eq:var-decomposition-2} becomes Eq. \ref{eq:var-decomposition-1} when the output distribution is Gaussian, where the mean and median will be the  same, (${q_{50\%}}_{\theta} = \mu_\theta$), and 
$({q_{66\%}}_\theta - {q_{33\%}}_\theta)/2$ will be equal to $\sigma_\theta$.

%For training the DCRNN ensemble, we adopted a randomization-based technique in which ensemble members run independently without interacting. The advantage of this strategy is that ensemble training can be executed on multiple compute nodes simultaneously.

%There are two type of ensemble approaches used widely 1) randomization-based approach ensemble like random forest where ensemble members run independently without interactions. 2) boosting-based approach where ensemble members fit sequentially one after another. We used randomization based approach for training ensemble DCRNN as it is better for simultaneous computation on different compute nodes. We randomly initialized the parameters of the $M$ DCRNN models.






==> UQ_DCRNN_ arxiv/5.results.tex <==
% \subsection{Negative log likelihood}
% We also use negative log-likelihood \cite{nix1994estimating} to capture predictive uncertainty. In the final layer, we modified the network to output two values, corresponding to the predicted mean and variance. We minimize the negative log-likelihood by treating the observed value as a sample from a Gaussian distribution with the predicted mean and variance.

% \begin{equation*}
%  -log p_{W} = \frac{1}{N} \mathlarger{\mathlarger{\sum}}_{j=1}^{N} \frac{1}{n} \mathlarger{\mathlarger{\sum}}_{i=1}^{n} \frac{log\sigma_W^2 (x_i)}{2} + \frac{(y_i - \mu_W (x_i))^2}{2\sigma_W^2(x_i)} + cst 
% \end{equation*}

% \TM{not finished yet}


%First, we write down our experimental setup here. 
In this section we extensively evaluate our proposed DCRNN-SQRUQ method and compare it with state-of-the-art UQ techniques proposed for DCRNN.
We conduct experiments on the METR-LA dataset, which contains speed profiles, given in miles per hour (mph), of 207 sensor locations collected from the loop detector on the highways of Los Angeles County. It contains time series data from March 1, 2012, to June 30, 2012, aggregated at 5-minute intervals, for a total of 34,272 timestamps. From the 4-month data, 70\%  (first 12 weeks approx.) is used for training, 10\% (1.7 weeks approx.) for validation, and 20\% (3.4 weeks approx.) for testing. %\PB{are these same for Rose's paper?} \TM{yes}. 
This dataset is widely used for benchmarking traffic forecasting techniques \cite{li2018dcrnn_traffic, mallick2020graph, zheng2020gman} %\PB{cite papers}
including the recent state-of-the-art UQ estimation work \cite{wu2021quantifying}. % \PB{cite}. 
The default hyperparameter configuration used for DCRNN is as follows: batch size -- 64; filter type -- dual/bidirectional random walk (captures both the upstream and the downstream traffic dynamic);  number of diffusion steps -- 2; RNN layers -- 2; RNN units per layer-- 64; optimizer -- Adam;  threshold for gradient clipping -- 5; initial learning rate -- 0.01; and learning rate decay -- 0.1. The adjacency matrix of the graph connectivity has been built by using the driving distance between the sensor locations. The DCRNN model uses the past 60 minutes of time series data at each node of the graph to forecast traffic for the next 5, 10, 15, ..., 60 minutes. 
To evaluate the performance, we use the same metrics used in the current state-of-the-art DCRNN UQ estimation work \cite{wu2021quantifying}. These metrics are the  mean absolute error (MAE), mean interval score (MIS), and Interval score. 
MAE is defined as
\begin{equation}\label{eq_mae}
%\begin{align*}
\text{MAE} =  \frac{1}{N} \mathlarger{\mathlarger{\sum}}_{j=1}^{N} \frac{1}{n} \mathlarger{\mathlarger{\sum}}_{i=1}^{n} | y_i - \hat{y}_i |,
%\end{align*}
\end{equation}
where $N$ is the total number of sensor locations and $n$ is the number of  timestamps for each sensor locations.
%\PB{where, say what N and n are}
% The RMSE can be defined as:
% \begin{align*}
% \text{RMSE} &= \sqrt{ \frac{1}{N}\sum_{i=1}^N ( y_i - \hat{y}_i )^2 }
% \end{align*}
MIS and interval scores are defined as
\begin{equation}\label{eq_mis}
\begin{array}{cc}
    \text{MIS}(q_u,q_l,q) &= \frac{1}{N} \mathlarger{\mathlarger{\sum}}_{j=1}^{N} \frac{1}{n} \mathlarger{\mathlarger{\sum}}_{i=1}^{n}  (q_{u_{ij}}-q_{l_{ij}}) \\
    & + \frac{2}{\rho} (y_{ij} - q_{u_{ij}}) \mathbb{1} \{y_{ij} > q_{u_{ij}}\} \\
    & + \frac{2}{\rho} (q_{l_{ij}} - y_{ij}) \mathbb{1} \{y_{ij} < q_{l_{ij}}\}
    \end{array}
\end{equation}


\begin{equation}\label{eq_interval}
\text{Interval} = \frac{1}{N} \mathlarger{\mathlarger{\sum}}_{j=1}^{N} \frac{1}{n} \mathlarger{\mathlarger{\sum}}_{i=1}^{n}  (q_{u_{ij}}-q_{l_{ij}}),
\end{equation}
where  $N$ is the total number of sensor locations and $n$ is the number of  timestamps for each sensor locations.
The estimated upper and lower quantiles $q_u$ and $q_l$ are the $(1-\frac{\rho}{2})$ and $\frac{\rho}{2}$ quantile for the confidence interval $(1-\rho)$, and $y$ is the observed value. %The interval would be 95 if the  forecasting quantiles are 0.25 and 0.975. 
%For example, if the confidence interval is 95\% or 0.95, then $(1-q) = 0.95$ and $q = 0.05$. The upper quantile $(1-\frac{q}{2}) = (1 - 0.05/2) = 0.975$ or 97.5\% and the lower quantile $\frac{q}{2} = 0.05/2 = 0.025$ or 2.5\%.
For example, if $q = 0.05$, then the upper quantile is $(1-\frac{q}{2}) = (1 - 0.05/2) = 0.975$ or 97.5\%,  the lower quantile is $\frac{q}{2} = 0.05/2 = 0.025$ or 2.5\%, and the confidence interval is $(1-q) = (1 - 0.05) = 0.95$ or 95\%.


Note that MIS defined in Eq.~\ref{eq_mis} penalizes for two factors: (1) a large interval width $(q_{u_{ij}}-q_{l_{ij}})$, and (2) the observed value being either higher or lower than the upper or lower quantiles. %\PB{what is threshold? do you the quantiles defined in the previous sentence}. 
MIS  focuses only on calculating intervals by examining the upper and lower quantiles. It does not taken into account the median/ mean prediction. For example, the upper quantile value is 63.33, the lower quantile value is 60.97, and the observed value is 58.87. Then, MIS is (63.33 - 60.97) + 2/0.05 (60.97 - 58.87) = 2.36 + 40* 2.1 = 82.36. If the observed value is 61.87, then the MIS is just the interval (63.33 - 60.97) = 2.36. 

%\PB{you have exlain this clearly}

%https://robjhyndman.com/hyndsight/m4competition/
The MIS score measures how narrow a given confidence interval defined by the quantiles is and whether the ground truth is within the interval or not. Additional details on this score can be found in \cite{gneiting2007strictly}. % \PB{cite} for additional details.
%GIL  - I  think  the citation is T. Gneiting, A. E.  Raftery. Strictly  proper scoring rules, prediction, and estimation. Journal of the American Statistical Association, Vol. 102 (March): 359-378. 

The experimental evaluation was conducted on a GPU-based cluster 
%name Cooley at the Argonne Leadership Computing Facility. This cluster has 
with 126 nodes. Each of them contains two 2.4 GHz Intel Haswell E5-2620 v3 CPUs and one NVIDIA Tesla K80 dual-GPU card (two K40 GPUs), enabling two model trainings per node.
%Each CPU has six cores, total 12 cores and 384 GB RAM per core.  
%Each GPU has two nodes, 12 GB RAM per GPU. Tesla K80 GPUs are used to run the DCRNN model for our experiments.
%\PB{not clear what do you mean by this?} \TM{means I run DCRNN in the GPU did not used the CPU }. 
The code was implemented in TensorFlow 2.4 and used Python 3.7.0.
We used SDV package (v0.14.0)~\cite{7796926} for fitting the GC models, where one-hot encoding was used for handling the categorical hyperparameter values.

%\subsection{Search space for hyperparameter search}
%Here we define search space for the hyperparameters configuration. 
For the hyperparameter search (HPS), we use the learning rate in the continuous range [.0001, 0.02], learning rate decay ratio in the continuous range [0.001, 0.02], filter type in the categorical range [Laplacian, random walk, dual random walk], batch size [8, 16, 32, 64, 128, 256], maximum diffusion steps [1, 2, 3, 4, 5], number of layers for the encoder  [1, 2, 3, 4, 5], number of layers for the decoder [1, 2, 3, 4, 5], number of RNN units per layer  [4, 5, 6,..,128], number of epoch  [20,21,...,100], and  threshold for gradient clipping [1,2,3,...,10] in the discrete range.


\subsection{Impact of scaling hyperparameter search on ensemble accuracy}

Here we show that scaling the HPS results in an increased number of high-performing hyperparameter configurations that can improve the quality of Gaussian copula model and the overall ensemble accuracy.

%study the scale the HPS and study its impact on the accuracy and uncertainty estimation. 
For the scaling experiments, we ran DeepHyper HPS runs with 10, 25, 50, and 100 workers, each with 
12 hours of wall time as the budget. We note that each compute node in the cluster can run up to 2 workers simultaneously. These runs resulted in 49, 108, 203, and 453 model evaluations, respectively. The default hyperparameter configuration achieved a validation SQR loss of $2.46$. Therefore, we consider the hyperparameter configurations as high  performing when they have a validation loss less than $2.46$.

%We analyzed the scaling with respect to GPUs utilization, number of high-performing hyperparameter configurations generated, and the impact on the performance of our proposed method DeepSQRUQ.
%We run hyperparameter searches on 10, 25, 50, and 100 GPUs, with 49, 108, 203, and 453 evaluations completed for each experiment, respectively. for each GPUs count.  

Figure \ref{fig_scaling} shows the cumulative number of high-performing configurations obtained by DeepHyper as a function of search time. We observe that the number of high-performing configurations increases almost linearly with the increase in the number of workers. In particular, with 100 workers, the search achieves 50 high-performing configurations within 6 hours, whereas the search with 50 workers takes 10 hours to reach that number. In 6 hours, the 100-worker search finds more high-performing configurations than the  25- and 10-worker  searches find. %\PB{the bar plot is redundant; remove the bar plot and add the numbers in the first plot directly}. 
The number of high-performing configurations obtained by 10-, 25-, 50-, and 100-worker searches is 23, 45, 98, and 172, respectively.

\begin{figure}[!ht]
\centering
   \includegraphics[width=\linewidth,height=0.5\linewidth]{images/hps_with_time.png}  
\caption{Hyperparameter configurations with validation loss less than 2.46 for different number of workers in DCRNN hyperparameter search. The plot shows that scaling hyperparameter search is critical for finding a large number of high-performing configurations.} %\PB{remove b; and add the numbers directly in the plot a; replace GPUs by workers in the legend}
\label{fig_scaling}
\end{figure}

%The bar plot in the Figure \ref{fig_scaling2} total number of high-performing configurations found for each GPUs count. Overall, the plots shows that scaling is important to find high-performing configurations.

\begin{figure}[ht]
    \centering
     \includegraphics[width=\linewidth,height=0.5\linewidth]{images/scale_val_los.png}  
\caption{Validation loss distribution of 100 models sampled from a Gaussian copula trained with HPS results with different workers.} %\PB{x-axis should be Number of workers used for the HPS}
\label{fig_scaling_val_loss}
\end{figure}

Next we selected a number of high-performing configurations from the DeepHyper HPS runs for generative modeling. For a given worker-count search run, we computed a 10\% quantile of the validation loss values of all hyperparameter configurations. We then selected the configurations that were less than or equal to that cut-off value. These configurations were used to fit a Gaussian copula (GC) model. We applied this procedure for each worker-count search run and denoted the resulting five GC models as GC-10, GC-25, GC-50, and GC-100. Table \ref{tab_GC_time} lists the time taken by each GC model to fit the configurations and sample new hyperparameter configurations from the distribution. We observe that time required for fitting the GC model and sampling from the model is negligible (less than 3 seconds for fitting and 0.04 second for sampling on a single CPU node). 
Once they were fitted, we sampled 100 new hyperparameter configurations from each GC model and trained all them simultaneously on 50 K80 nodes (two model training per node). 

\begin{table}
\centering
\begin{tabular}{|l|l|l|} 
\cline{2-3}
\multicolumn{1}{l|}{} & Fit time (sec) & Sample time (sec)  \\ 
\hline
GC-10~                & 2.57           & 0.030              \\ 
\hline
GC-25                 & 2.82           & 0.031              \\ 
\hline
GC-50                 & 2.89           & 0.032              \\ 
\hline
GC-100                & 2.96           & 0.038              \\
\hline
\end{tabular}
\caption{Time taken to fit the configurations to the GC models (GC-10, GC-25, GC-50, and GC-100) and sample 100 configurations from the trained GC models.}
\label{tab_GC_time}
\end{table}
 
Figure \ref{fig_scaling_val_loss} shows a box plot of the validation loss distribution of 100 trained models from GC-10, GC-25, GC-50, and GC-100. The results clearly show that the validation loss significantly decreases as we move to GC models trained with a larger number of workers. The median values of the validation loss distributions are 3.24, 3.0, 2.77, and 2.47 for GC models trained with 10-, 25-, 50-, and 100-workers HPS results, respectively.

For model selection, we selected the top 25 models from the generated 100 based on the validation loss. The number 25 is motivated by the fact that the state-of-the-art SG-MCMC method used 25 posterior sample models from the trained model. 

We also compared the validation loss distributions of (1) all the hyperparameter configurations in the HPS run, (2) 10\% quantile subset of the HPS run used for training the  GC-100 model, (3) 100 models from GC-100, and (4) the top 25 of 100 models from GC-100.
%hyperparameter configurations that were used to train the GC model, the 100 newly sampled hyperparameter configurations from the GC model, and the top 25 hyperparameter configurations selected based on the validation loss values. 
The results are shown in Figure \ref{fig_gc}. 
%The left most box plot shows the distribution of the validation loss from 10\% quantile of actual hyperparameter configurations. The next box plot shows the distribution of the validation loss from 100 models trained on synthetic hyperparameter configurations. Next two box plots show the distribution of the validation loss from top 25\% and 50\% models from the model ensemble of 100 synthetic hyperparameter configurations. The  median of the distribution is shown as the horizontal line in the middle of the box. 
The results show that the validation loss distribution achieved by the top 25 models is superior to the hyperparameter values found by the search alone. Moreover, using all 100 models from the GC model results in a validation loss distribution that is better than that of HPS run. The strategy of generating models from GC and selecting a subset from them seems a good strategy. We expect that by generating a large number of high-performing configurations by scaling HPS further and/or by using faster GPUs, we can train better GC models, which will result in overall improvement in the ensemble validation loss distribution.  

\begin{figure}[ht]
  \centering
  % include first image
   \includegraphics[width=\linewidth,height=0.5\linewidth]{images/syn_hps.png}  
  \caption{Validation loss distributions of four settings: (1) all the hyperparameter configurations in the HPS run with 100 workers, (2) 10\% quantile subset of the HPS run used for training the GC-100 model, (3) 100 models from GC-100, and (4) the top 25 of the 100 models sampled from GC-100} %\PB{update the x-axis label to: all, 10\% quantile subset, 100 model from GC, top 25 from GC }} % \PB{remvove the last box}}
  \label{fig_gc}
\end{figure}

Using the selected 25 models, we performed  inference on the test data and computed the test loss. The results are shown in Figure \ref{fig_scaling_test_loss}. We observe that the 25 models generated with a larger number of workers for the HPS significantly reduce the test loss. The trend is similar to the validation loss distribution with 100 models. The medians of the distribution are 3.96, 3.89, 3.45, and 2.8 for 10, 25, 50, and 100 workers, respectively.  The findings lead us to conclude that when conducted on a large number of workers, HPS yields better configurations, which result in improved overall predictive accuracy of the ensembles.


%Thereafter, we selects model for top 25\% quantile of the validation loss and plot the distribution of the test loss in the . The test loss show same trend as the validation loss. The plot shows that the test loss for the HPS decreases as the number of workers rises. 

\begin{figure}[ht]
    \centering
     \includegraphics[width=\linewidth,height=0.5\linewidth]{images/scale_test_loss.png}  
\caption{Test loss distribution of top 25 out of 100 models sampled from Gaussian copula trained with results from HPS with different workers.} % \PB{x-axis: number of workers used for HPS}}
\label{fig_scaling_test_loss}
\end{figure}

\begin{comment}
\begin{figure}[ht]
  \centering
  % include first image
   \includegraphics[width=\linewidth,height=0.5\linewidth]{images/hps_val_loss.png}  
  \caption{Objective function obtain from the hyperparameter configurations generated over time. The red line depicts the objective function for default hyperparameter configurations.}
  \label{fig_hps}
\end{figure}

HPS was carried out across 100 workers on the Cooley GPU cluster. The job ran for the maximum of 12 hours of wall time and generated 453 configurations. The objective function is used to select high-performing configurations. The evolution of the objective function over time is depicted in Figure \ref{fig_hps}. At first, the algorithm chooses random configurations. Each configuration is evaluated by training the model and then computing the error on the validation dataset. The algorithm learns the relationship between hyper parameter configurations and the objective function over time and generates more promising configurations. The objective function for default hyperparameter configurations is depicted in the figure \ref{fig_hps} by the red line.
\end{comment}




\subsection{Uncertainty estimation and comparison with the state-of-the-art}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\begin{scriptsize}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
T                        & Metric       & Point & Bootstrap  & Quantile & SQ  & MIS & MC Dropout  & SG-MCMC & {\bf DCRNN-SQRUQ}  \\ \hline
\multirow{4}{*}{15 mins} & MAE (mean)   & 2.38  & 2.63          & 2.43         & 2.67   & 2.63   & 2.47           & 2.32        & {\bf 2.21} \\ \cline{2-10} 
                         & MAE (median) &       &               &              &        &        &                &             & {\bf 2.20}         \\ \cline{2-10} 
                         & MIS          &       & 39.76         & {\bf 18.32}       & 29.04  & 18.26  & 27.61          & 32.21       & 24.79      \\ \cline{2-10} 
                         & Interval     &       & {\bf 5.8}           & 12.42        & 8.38   & 12.46  & 8.99           & 8.73        & 8.29           \\ \hline
\multirow{4}{*}{30 mins} & MAE (mean)   & 2.73  & 3.19          & 2.79         & 3.1    & 3.08   & 2.94           & 2.54        & {\bf 2.44}\\ \cline{2-10} 
                         & MAE (median) &       &               &              &        &        &                &             & {\bf 2.45}       \\ \cline{2-10} 
                         & MIS          &       & 38.48         & 21.54        & 40.93  & {\bf 21.09}  & 33.38          & 31.87       & 27.4       \\ \cline{2-10} 
                         & Interval     &       & {\bf 7.86}         & 13.48        & 8.37   & 13.99  & 11.1           & 12.62       & 10.53       \\ \hline
\multirow{4}{*}{60 mins} & MAE (mean)   & 3.14  & 3.99          & 3.19         & 3.75   & 3.65   & 3.7            & 3           & {\bf 2.83} \\ \cline{2-10} 
                         & MAE (median) &       &               &              &        &        &                &             & {\bf 2.80}    \\ \cline{2-10} 
                         & MIS          &       & 38.58         & 25.74        & 60.56  & {\bf 24.33}  & 43.11          & 30.35       & 29.33     \\ \cline{2-10} 
                         & Interval     &       & 11.65         & 14.5         & {\bf 8.38}   & 15.55  & 14.46          & 18.79       & 12.34        \\ \hline
\end{tabular}
\caption{Performance comparison of different UQ methods}
\label{tab_comp}
\end{scriptsize} 
\end{table*}

In this section we compare the uncertainty estimates from our proposed DCRNN-SQRUQ with several other DCRNN UQ techniques that were used in a recent study \cite{wu2021quantifying} and show that our method outperforms all other methods. For the experimental comparison, we adopt the same setup in terms of error metrics, forecasting horizons, and confidence interval as described in \cite{wu2021quantifying}.

%Using SQR, a single DCRNN model is trained using SQR loss function and the prediction is performed on 80\% confidence interval (10\% , 50\%, and 90\% quantile), 90\% confidence interval (5\%, 50\%, and 95\%), 95\% confidence interval (2.5\% 50\%, and 97.5\% quantile). For each confidence interval, we calculate MAE, and MIS from the prediction in three quantiles. 

%We estimate the epistemic uncertainty captured using the deep ensemble method. We train 100 DCRNN models with different random seeds and all ensemble members are trained simultaneously. The dataset and hyperparameter configurations are the same for all the 100 models. After training, we forecast the speed for 15 minutes, 30 minutes, and 1 hour and calculate the mean speed and standard deviation for each timestamp of all sensors. Farther, the mean speed is used to calculate the error metrics such as MAE, RMSE, and MIS.  


%We compare the performance of our DeepSQRUQ deep ensemble method with other methods of uncertainty estimation \cite{wu2021quantifying}. 
The uncertainty estimation techniques reported in \cite{wu2021quantifying} are as follows.
(1) Bootstrap \cite{efron2016computer}: This method randomly samples 50\% of training data points to train DCRNN  model. Prediction is performed on the entire test dataset, and 25 samples are collected in order to calculate mean predictions and confidence intervals.
(2) Quantile \cite{koenker2005quantile}: This method uses pinball loss for DCRNN, and the prediction is performed for three different quantiles 2.5\%, 50\%, and 97.5\% (95\% confidence interval).
(3) Spline quantile regression (SQ) \cite{gasthaus2019probabilistic}: This method models the quantile functions using linear splines and optimizes the continuous ranked probability score as a loss function. 
%11 parameters \PB{not clear what do you mean by this?} are used to make the quantile function for every point prediction. \TM {removed it} 
(4) Mean Interval Score  \cite{wu2021quantifying}: MIS is directly used in the loss function along with MAE, and a multiheaded model is used to jointly output the upper bound, lower bound, and prediction for a given input. 
(5) Monte Carlo  Dropout \cite{gal2016dropout}: This method uses the algorithm develops by Zhu et al. \cite{zhu2017deep}. A 5\% random drop rate is used during the testing time over 50 iterations to get a stable prediction.
(6) Stochastic Gradient Markov Chain Monte Carlo (SG-MCMC) \cite{ma2015complete}: This is the current state of the art Bayesian neural network for DCRNN and uses a subsampling technique to minimize the cost of Markov chain Monte Carlo (MCMC) per iteration. A Gaussian prior $\mathcal{N}$(0, 0.4) with randomly initialization of $\mathcal{N}$(0, 0.2) is used for the model parameters. %\PB{for what?}. 
The mean and confidence intervals are obtained by averaging from 25 posterior model samples.

The comparison results are shown in the Table~\ref{tab_comp}. The results of the six methods (Bootstrap, Quantile, SQ, MIS, MC Dropout, SG-MCMC) are taken directly from \cite{wu2021quantifying}. The performance of each method is evaluated by using the error metrics MAE and MIS (95\% confidence interval). The comparison is done on three different forecasting horizons: 15 minutes, 30 minutes, and 60 minutes. 

%For our proposed DCRNN-SQRUQ method, we construct an ensemble of 100 models trained using high-performing hyperparameter configurations generated from Gaussian copula. The validation loss from the 100 models are used to select top 25\%, 50\%, and 100\% models. To perform a head-to-head comparison with the previous methods (The final result is calculated using 25 posterior samples by SG-MCMC and 25 samples by bootstrap), we compare the results of top 25\% quantile of our method. We compute the mean and median MAE values derived from the ensemble of multiple models. 

The results show that our DCRNN-SQRUQ method outperforms the state-of-the-art SG-MCMC method and a number of other UQ methods. The mean and the median MAE of our DCRNN-SQRUQ shows a better prediction accuracy in MAE than does SG-MCMC across all three forecasting horizon. Moreover, the MIS score and interval (defined in Eqs. \ref{eq_mis} and \ref{eq_interval})  %\PB{where did you define this metric?} \TM{referd the equations}
show that our method achieves a low MIS score and interval with a narrow interval compared with other techniques. An exception is for the MIS method that directly minimizes the MIS score in the loss function;  as expected, it achieves the best MIS performance. However, the prediction accuracy and interval score of DCRNN-SQRUQ are better than those found by MIS. 
Overall, our proposed DCRNN-SQRUQ is more robust in prediction accuracy and achieves MIS and interval scores that are better than the state of the art SG-MCMC method.

%sidrom that, our method achieves better MIS score with a narrow interval than other techniques. %\PB{what about the interval score?} \TM{added interval score}
%\PB{poor writing in this section}
%\subsection{High-performing configurations generation} 
%Here we generate High-performing configurations using Gaussian copula. We choose the top 10\% quantile of hyperparameter configurations, which is 46  configurations, based on the objective function. We used a Gaussian copula model to represent the joint distribution of diffident hyperparameter configurations and objective functions. Then, to generate high-performing configurations, we sample from a multivariate Gaussian distribution. We sample 100 synthetic hyperparameter configurations from the distribution and train 100 DCRNN models with those configurations.  The 


%For aleatoric uncertainty, we compare SQR with quantile, SQ, and MIS.  For 15 minutes horizon, deep ensemble achieves MAE of 2.28 $\pm$ 1.02 and RMSE 4.16 $\pm$ 1.31, which are better than other techniques. Similarly, for 30 minutes horizon, the performance of SQR is comparable with quantile in terms of MAE (2.76 $\pm$ 1.17) and RMSE (6.05 $\pm$ 2.06). On the other hand, for 60 minutes horizon, quantile achieved better performance compare to SQR. MIS method achieved a better interval score (80\%, 90\%, 95\%) as the model optimize MIS in loss function along with the MAE. The performance of SQR is  comparable with quantile regression. The advantage of SQR is that one SQR model can jointly estimate all the quantiles of the target where as quantile regression estimates a given quantile of target. SQR is capable to estimate the non-Gaussian, skewed, asymmetric, multimodal, and heteroskedastic noise of data \cite{tagasovska2018single}. For epistemic uncertainty, we compare the deep ensemble technique with bootstrap, MC-Dropout, and SG-MCMC. For 15 minutes horizon, deep ensemble achieves MAE of 2.16 $\pm$ 0.91 and RMSE 3.87 $\pm$ 1.40, which are better than other techniques. Similarly, for 30 minutes horizon, deep ensemble performs better than others in terms of MAE (2.93 $\pm$ 1.30) and RMSE (5.34 $\pm$ 2.04). On the other hand, for 60 minutes horizon, SG-MCMC achieved better performance compared to others. The performance of deep ensemble and SG-MCMC are comparable. The deep ensemble can be scale very easily. $M$ different model can be distributed over $M$ node of the cluster and run all models simultaneously without interaction, whereas data/model parallel training of SG-MCMC is not straightforward. 

%The performance of deep ensemble and SG-MCMC are comparable. But, in case of large dataset and imitated compute per node does not impact on deep ensemble as the model size does not change in terms of number of parameters. Whereas, SG-MCMC (like all Bayesian methods) are computationally expensive as those increase the number of model parameter of the model as the network weights come from a prior distribution. Farther, deep ensemble can be easily distributed over $M$ node of cluster as $M$ different model can run simultaneously without interaction, whereas data/model parallel learning of SG-MCMC is not straightforward. 

% We also select the top models for deep ensemble and shows the results. We select top 5, 25, 50, 75, and 100 models based on MAE of the 60 minutes predictions. The result  in the table \ref{tab_top_model} shows the  MAE and standard deviation of top models. The result shows that the MAE of the top 5 model is 3.07 $\pm$ 1.51, which is quite comparable with SG-MCMC method. This shows that the ensemble result can be improved further by  discarding the models which are not learnt well.


% \begin{table} [!ht]
% \centering
% \begin{tabular}{|l|l|} 
% \hline
% \bf{Top Models} & \bf{MAE}   \\ 
% \hline
% 5 models   & 3.07 $\pm$ 1.51 \\ 
% \hline
% 25 models  & 3.18 $\pm$ 1.53 \\ 
% \hline
% 50 models  & 3.24 $\pm$ 1.54 \\ 
% \hline
% 75 models  & 3.30 $\pm$ 1.56 \\ 
% \hline
% 100 models & 3.36  $\pm$ 1.57\\
% \hline
% \end{tabular}
% \caption{Performance of the top models}
% \label{tab_top_model}
% \end{table}





% \subsection{Impact of the data in uncertainty estimation}
% %Aleatoric uncertainty occurs due to irreducible uncertainty of data. On the other hand, epistemic uncertainty occurs due to uncertainty associated with the estimation of model parameters and limited knowledge about the data generating system, which creates a discrepancy between the model and distribution of the data generation. Hence, 
% Aleatoric or data uncertainty is irreducible by adding more data whereas epistemic or model uncertainty can be reduced by adding more data (shown by Liu et al. \cite{liu2019accurate}). In this section, we empirically validate the effect of dataset size on aleatoric and epistemic uncertainty. Our original METR-LA training set had 12 months of training data. We further reduce the training dataset to 8 months and 4 months and keep the testing and validation data untouched. In this manner, we create 3 datasets by varying training data size. 3 datasets are used to
% estimate the aleatoric uncertainty using the SQR method and epistemic uncertainty using the deep ensemble method. The evaluation is done using the error metrics MAE and RMSE over 15 minutes, 30 minutes, and 60 minutes forecasting horizon. %using 12 weeks, 8 weeks, and 4 weeks of training data.

% Table \ref{tab_data_alea} shows the impact of the dataset size on aleatoric uncertainty. In 60 minutes forecasting horizon, the MAE and std remain almost the same 3.49 $\pm$ 1.73 (RMSE 6.41 $\pm$ 1.89), 3.52 $\pm$ 1.68 (RMSE 6.40 $\pm$ 1.84) and 3.51  $\pm$ 1.74 (RMSE 6.45 $\pm$ 1.86) as the training dataset decreased from 12 months to 8 months, and 4 months. 15 minutes and 30 minutes horizons show a similar trend. Overall, the results show that the aleatoric uncertainty does vary significantly with the size of the dataset. On the other hand, table \ref{tab_data_epis} shows the impact of the dataset size on epistemic uncertainty.  In 60 minutes forecasting horizon, the MAE and std increase from 3.29 $\pm$ 1.58 (RMSE 6.74 $\pm$ 2.62) to 3.72 $\pm$ 1.82 (RMSE 9.03 $\pm$ 2.78) and 4.10 $\pm$ 2.10 (RMSE 10.92 $\pm$ 2.94) as the training dataset decreased from 12 months to 8 months, and 4 months. A similar trend can observe in 15 minutes and 30 minutes forecasting horizon. The results show that the increase in the dataset size help to reduce the epistemic uncertainty of the model.

% \begin{table}[]
% \begin{tabular}{l|l|l|l|l|}
% \cline{2-5}
%                                                 & Metric & 15 mins                        & 30 mins         & 60 mins         \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{12 Weeks}} & MAE    & 2.28 $\pm$ 1.02                & 2.76 $\pm$ 1.15 & 3.49 $\pm$ 1.73 \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                          & RMSE   & 3.49 $\pm$  1.06               & 5.26 $\pm$ 1.27 & 6.41 $\pm$ 1.89 \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{8 Weeks}}  & MAE    & 2.30 $\pm$ 1.01               & 2.75 $\pm$ 1.08 & 3.52 $\pm$ 1.68 \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                          & RMSE   & 3. 48 $\pm$ 1.05              & 5.13 $\pm$ 1.19 & 6.40 $\pm$ 1.84 \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{4 Weeks}}  & MAE    & 2.34 $\pm$ 1.00                & 2.72 $\pm$ 1.17 & 3.51 $\pm$ 1.74 \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                          & RMSE   & 3.49 $\pm$ 1.08 & 5.14 $\pm$ 1.29 & 6.45 $\pm$ 1.86 \\ \hline
% \end{tabular}
% \caption{Effect of dataset reduction on Aleatoric uncertainty. Aleatoric uncertainty does not get impacted by the dataset size.}
% \label{tab_data_alea}
% \end{table}


% \begin{table}[]
% \begin{tabular}{l|l|l|l|l|}
% \cline{2-5}
%                                                 & Metric & 15 mins         & 30 mins         & 60 mins          \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{12 Weeks}} & MAE    & 2.16 $\pm$ 0.91 & 2.93 $\pm$ 1.30 & 3.36 $\pm$ 1.57  \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                          & RMSE   & 3.87 $\pm$ 1.40 & 5.34 $\pm$ 2.04 & 6.74 $\pm$ 2.62  \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{8 Weeks}}  & MAE    & 2.39 $\pm$ 1.03 & 3.33 $\pm$ 1.49 & 3.72 $\pm$ 1.82  \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                          & RMSE   & 5.05 $\pm$ 1.69 & 6.34 $\pm$ 2.43 & 9.03 $\pm$ 2. 78 \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{4 Weeks}}  & MAE    & 2.87 $\pm$ 1.28 & 3.50 $\pm$ 1.76 & 4.10 $\pm$ 2.10  \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                          & RMSE   & 5.53 $\pm$ 1.92 & 7.97 $\pm$ 2.57 & 10.92 $\pm$ 2.94 \\ \hline
% \end{tabular}
% \caption{Effect of dataset reduction on Epistemic uncertainty. Epistemic uncertainty increases with smaller dataset.}
% \label{tab_data_epis}
% \end{table}

%\subsection{Aleatoric and Epistemic Uncertainty Estimate}




\subsection{Uncertainty vs traffic dynamics}
Here we estimate aleatoric and epistemic uncertainty using DCRNN-SQRUQ and investigate the relationships between the traffic dynamics and the estimated uncertainty measures. According to this analysis, increased traffic dynamics produced by fast changes in traffic behavior result in high aleatoric and epistemic uncertainty. Currently, none of the existing UQ methods developed for DCRNN provide separate aleatoric and epistemic uncertainties. 


Traffic dynamics describe the change in traffic behavior observed by the variability of the traffic speed. High dynamics indicate instability in the speed caused by rapid change of traffic behavior, whereas low dynamics indicate stable behavior of the traffic. 
The traffic dynamics at a given sensor location can be measured by the coefficient of variation (COV) \cite{mallick2020graph} of the time series data (speed). The COV becomes large (small) when the variations/change in the speed values are high (low). To measure COV, we calculated the mean ($\mu$)  and standard deviation ($\sigma$) of the speed of each sensor location over the entire timeline. The COV is estimated by $\sigma$/$\mu$. Afterwards, the COV on METR-LA dataset are binned in four ranges: (1) $0.2 <$ COV $< 0.3$;  (2) $0.3 <$ COV $< 0.4$; (3) $0.4 <$ COV $< 0.5$; and (4) $0.5 <$ COV. The binning helps us identify the sensor location with low to high traffic dynamics. Of a total of 207 sensor locations, 34 locations have COV between 0.2 and 0.3,  120 locations have  COV between 0.3 and 0.4,  42 locations have COV between 0.4 and 0.5, and 11 locations have COV more than 0.5.

\begin{figure}[ht]
  \centering
   \includegraphics[width=\linewidth,height=0.5\linewidth]{images/cov_ale.png}  
\caption{Coefficient of variation of the sensors  binned into four categories. Box plots depict the aleatoric uncertainty estimation for each bin on the 15-, 30-, and 60-minute forecasting horizons using DCRNN-SQRUQ.}
\label{fig_cov_ale}
\end{figure}

\begin{figure}[ht]
  \centering
   \includegraphics[width=\linewidth,height=0.5\linewidth]{images/cov_epi.png}  
\caption{Coefficient of variation of the sensors  binned into four categories. Box plots depict the epistemic uncertainty estimation for each bin on the 15-, 30-, and 60-minute forecasting horizons using DCRNN-SQRUQ.}
\label{fig_cov_epi}
\end{figure}

We estimate the aleatoric and epistemic uncertainty using  Eq.~\ref{eq:var-decomposition-2}. The aleatoric uncertainty is the mean of the prediction variance of the 2.5\% and 97.5\% quantile over the top 25 models selected from the ensemble. 
For each sensor location we now have the COV value and the aleatoric uncertainty measure.  We separate the sensor locations based on the COV values into the four bins mentioned above and plot the distribution of aleatoric uncertainty across three forecasting horizons in box-and-whisker plot in Figure \ref{fig_cov_ale}.  We  have three forecasting horizons and four COV bins, for a total of 12 box plots per figure.
%The  median of the distribution is shown as the horizontal line in the middle of the box. The ends of each box are 25\% (bottom) and 75\% (top) quantiles of the distribution. 
Across all the COV bins we can observe that 25\%, median, and 75\% quantiles of the aleatoric uncertainty increase with the increasing COV values. The box plots for the 15-, 30-, and 60-minute forecasting horizons show a similar trend. This result indicates that the aleatoric uncertainty is high on the sensor locations with high traffic dynamics or COV values. Since the aleatoric  uncertainty is irreducible,  we cannot mitigate it. In a proactive traffic management system, however, aleatoric uncertainty can be used to estimate  worst-case traffic management and planning.




\begin{figure}[!t]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth,height=0.5\linewidth]{images/cov_23.png}  
  \caption{COV between 0.2 to 0.3}
  \label{fig_plot1}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth,height=0.5\linewidth]{images/cov_34.png}  
  \caption{COV between 0.3 to 0.4}
  \label{fig_plot2}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth,height=0.5\linewidth]{images/cov_45.png}  
  \caption{COV between 0.4 to 0.5}
  \label{fig_plot3}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth,height=0.5\linewidth]{images/cov_5.png}  
  \caption{COV above 0.5}
  \label{fig_plot4}
\end{subfigure}
\caption{60-min-ahead traffic forecasting on four sensors selected from 4 COV bins. The aleatoric uncertainty or 95\% prediction interval is shown in yellow shade, and the epistemic uncertainty is shown in blue shade.}
\label{fig_plot}
\end{figure}


Next, we estimate the epistemic uncertainty by using Eq. \ref{eq:var-decomposition-2}. Epistemic uncertainty measures the variance of the mean across top 25 models selected from the ensemble. Similar to the aleatoric uncertainty, we separate the sensor locations based on COV values into  four bins and plot the distribution of epistemic uncertainty across three forecasting horizons in box-and-whisker plots in Figure \ref{fig_cov_epi}. A similar trend can be observed here: the epistemic or  model uncertainty increases for the sensor locations having high COV value or traffic dynamics. 
The epistemic uncertainty for 60-minute forecasting is high for COV $> 0.5$ (9th box in the Figure \ref{fig_cov_epi}). The predictive uncertainty of the model is high due to the high traffic dynamics. Therefore, we recommend performing 15-minute forecasts for those sensor location where COV $> 0.5$ (11 sensors belong to this bin). The 15-minute forecast (7th box in Figure \ref{fig_cov_epi}) has a median of the distribution of the epistemic uncertainty below 10. Similarly, uncertainty is high for 60-minute forecasting in the COV bin between 0.4 to 0.5. Hence, we recommend  performing 30-minute forecasting for those sensor locations (42 sensors belong to this bin). The ability to provide these uncertainty measures and consequent recommendations is crucial to putting these models into practice. Limiting the forecasting horizon for highly dynamic sensors will stabilize the DCRNN prediction and minimize the risk of using the forecasting results for crucial decision making. 



% We also examine the relationship of the MAE and std with the COV values in case of aleatoric uncertainty estimated by SQR. The plot in Figure \ref{fig_mean_cov_ale} shows the distribution of MAE and Figure \ref{fig_std_cov_ale} shows the distribution of std. 
% For each forecasting horizon, we can observe that 25\%, median, and 75\% of the MAE and std increase as we go from COV between 0.2 \& 0.3 to COV $>$ 5.
% This shows that the aleatoric uncertainty also increases as the traffic dynamic increases. 

% \TM{I will change the order of aleatoric and epistemic here}
% Now, for epistemic uncertainty, we examine the relationship of the MAE and standard deviation (std) with the COV values. Using deep ensemble we perform prediction over 100 models.From those 100 predictions, we calculate the mean and standard deviation. Afterwards, the means prediction is used to calculate MAE over three (15, 30, and 60 minutes) forecasting horizon. Now, for each sensor location we have the COV value, MAE and std.  We segregate the sensor locations based COV values into 4 bins mentioned above. For each bin, we plot the distribution of MAE and std of three forecasting horizon in box-and-whisker. The ends of each box are 25\% (bottom) and 75\% (top) quantiles of the distribution, the  median of the distribution is shown as the horizontal line in the middle of the box, the two vertical lines on the two sides of the whisker represent 5\% and 95\% of the distribution, and the diamonds mark the outliers of the distribution.
% The plot in Figure \ref{fig_mean_cov} shows the distribution of MAE and Figure \ref{fig_std_cov} shows the distribution of std.
% We are having 3 forecasting horizon and 4 COV bins, total 12 box plot per figure.
% In all COV bin, we can observe that 25\%, median, and 75\% of the MAE and std increase with the increasing horizon. This phenomena shows that model error and the deviation of the prediction increase with the forecasting horizon.  
% Now, if we see the 60 minutes forecast across all COV bins, we can observe an increase in the 25\%, median, and 75\% of the MAE and std values with the increasing COV values. The box plot for 15 and 30 minutes shows similar trend. 
% This phenomena indicate that epistemic uncertainty increases as the traffic dynamic increases. 
% In case of 60 minutes prediction and COV $> 5$ (9$^{th}$ box in the Figure \ref{fig_mean_cov}, and \ref{fig_std_cov}), the median of MAE is above 6 mph and the std is above 1.5. The predictive uncertainty of the model is high due to high traffic dynamic. As the uncertainty is high for 60 minutes forecast, we recommend to perform 15 minutes forecast for those sensor location where COV $> 5$ (total 11 sensors belong to this bin). The 15 minutes forecast (7$^{th}$ box in the \ref{fig_mean_cov}, and \ref{fig_std_cov}) has median of MAE below 3 mph and std below 1.0 which are similar to the average error of the sensors. Similarly, 60 minutes prediction is uncertain in the COV bin between 0.4 to 0.5. Hence, we recommend to perform 30 minutes forecasting for those sensor locations (total 42 sensors belong to this bin). Limiting the forecasting horizon for highly dynamic sensor will stabilize the DCRNN prediction and minimize the risk of using the forecasting results for crucial decision making. \TM{here I can add the plots for 15min and 30 minutes if that help}


\begin{figure}[!t]
\centering
   \includegraphics[width=\linewidth,height=0.5\linewidth]{images/daily_ale.png}  
\caption{Time series data for sensor ID: 716960 over multiple days demonstrating the variability in the data. The aleatoric uncertainty on top of the daily variation indicates how well DCRNN-SQRUQ captures the variability.}
\label{fig_high_ale}
\end{figure}



Further, we plot 4 sets of time series data taken from 4 different COV bins in Figure \ref{fig_plot}. Each plot contains the observed and predicted timeseries data, and the epistemic and aleatoric uncertainty intervals estimated by our proposed method DCRNN-SQRUQ methods. The results shown in the Figure \ref{fig_plot} are for the 60-minute forecasting horizon. 
The epistemic uncertainty interval is calculated by using the 2.5\% and 97.5\% quantiles of the median prediction of the top 25 models - shown in blue. 
The aleatoric uncertainty intervals are the medians of the 2.5\% and 97.5\% quantile of the top 25 models- shown in yellow. 
Figure \ref{fig_plot1} shows the sensor location with the lowest COV value (between 0.2 and 0.3). Traffic behavior does not change rapidly in this COV bin. Hence, the interval band is narrow for both of the uncertainty measures. Figure \ref{fig_plot2} shows the sensor location with COV value between 0.3 and 0.4. Traffic dynamics are higher compared with the previous bin. 
Both the aleatoric and epistemic uncertainty measures are high around 9 am and 3 pm. The traffic dynamic increases more in Figure \ref{fig_plot3}, and the uncertainty band becomes even wider here.  Epistemic uncertainty estimates are high during the  drop/rise in traffic speed. 
In contrast, aleatoric uncertainty is high around 6  am, 9 am, 12 pm, 
and 11 pm. Specifically, during 9 am the uncertainty is high but the traffic is  stable. This uncertainty is coming from the data. Therefore, to validate it, we plot the timeseries data of the same sensor (sensor ID: 716960) over multiple days in box-and-whisker plot shown in the Figure \ref{fig_high_ale}. The results show huge variation in the speed profile during 3 am, 9 am, 12 pm, and 11 pm. We also plot the aleatoric uncertainty on top of the daily variation of the data. We see that our uncertainty measure covers the variation in the data. This explains the high uncertainty at 9 am in  Figure \ref{fig_plot3}. Likewise, the traffic dynamics increase more in  Figure \ref{fig_plot4} where the COV is greater than 0.5. The aleatoric uncertainty is high from 3 am to 7 am because of the variety of patterns  in the data. The epistemic uncertainty is high  during the drop/rise of traffic speed, which is difficult for the model to capture.
% high_ale





==> UQ_DCRNN_ arxiv/6.conclusion.tex <==
We developed DCRNN-SQRUQ, a scalable Gaussian assumption-free ensemble-based uncertainty quantification for traffic forecasting for spatial temporal graph neural networks. DCRNN-SQRUQ it employs simultaneous quantile regression loss for DCRNN, Bayesian hyperparameter search, generative modeling with a Gaussian copula mode, ensemble training, and variance decomposition for Gaussian quantile regression ensembles. 
DCRNN with SQR effectively captures  well-calibrated forecasting intervals. The Bayesian optimization-based scalable hyperparameter search efficiently finds the most promising hyperparameter configuration. We also showed that scaling the hyperparameter search is important for finding promising hyperparameter configurations and for improving the forecasting accuracy of the ensembles. The Gaussian copula generative model is inexpensive yet efficient in generating more high-performing hyperparameter configurations from promising hyperparameter configurations found in a hyperparameter search. Furthermore, we developed a variance decomposition methodology for DCRNN ensembles with SQR loss function and use it for estimating the aleatoric (data) uncertainty and epistemic (model) uncertainty.


We demonstrated that our approach outperformed the state-of-the-art Bayesian neural network method and a variety of other frequentist uncertainty techniques.
%our proposed method outperforms a Bayesian and and five frequentist uncertainty measurement techniques: bootstrap, quantile regression, spline quantile regression, Monte Carlo dropout, and SG-MCMC.
%GAIL  - that is only five - what one is left out?
Experiments on a real-world dataset showed that our method is robust in mean predictions and effective in capturing data variations. 
In addition, we investigated the relationship between aleatoric/epistemic uncertainty and traffic dynamics. The analysis showed that increased traffic dynamics caused by rapid changes in traffic behavior resulted in high aleatoric and epistemic levels. Because aleatoric uncertainty is irreducible, it can be used for worst-case traffic planning in proactive traffic management. The epistemic uncertainty can be used to identify the limitations of the model and appropriate location-specific forecasting horizons. Currently, no other UQ method can provide separate aleatoric and epistemic uncertainty estimates for the DCRNN and, in general, for any other traffic forecasting methods. From a practitioner perspective, it provides a mechanism for reducing the forecasting horizon when the uncertainty measure is too high. This is very important for reducing the risk of using the model in real-world decision making.

The key advantages of our approach are generality and scalability. Our proposed approach for building model ensembles is based on a scalable hyperparameter search and computationally inexpensive generative modeling. In principle, we can apply our UQ approach to any neural network models. This involves taking the default neural network architecture, using simultaneous quantile regression loss, running hyperparameter search, training a generative model from the hyperparameter search runs, performing model selection, and decomposing the uncertainty estimates. The scalability of the approach is derived from scalable hyperparameter search and scalable ensemble training. Both phases provide improvement with respect to ensemble predictive accuracy and uncertainty estimation. 

Our future work will include (1) application of the proposed UQ methods for various spatial and temporal forecasting neural network models; (2) comparison with other forms of Bayesian neural networks; (3) advanced generative modeling with autoencoders; and (4) uncertainty-informed traffic planning using reinforcement learning.

\clearpage

%We have demonstrated our approach on a benchmark dataset.  We plan to extend our approach for large-scale forecasting. Moreover, we plan to work on approaches to effectively utilize the uncertainty measure for proactive traffic planning in traffic management centers. 


==> UQ_DCRNN_ arxiv/extra.tex <==
\begin{table*}[!ht]\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
T                        & Metric        & DCRNN & Deep Ensembles           & Bootstrap & Quantile & SQ    & MIS            & MC Dropout & SG-MCMC       \\ \hline
\multirow{8}{*}{15 mins} & MAE           & 2.77  & \textbf{2.16 $\pm$ 0.91} & 2.63      & 2.43     & 2.67  & 2.63           & 2.47       & 2.32          \\ \cline{2-10} 
                         & RMSE          & 5.38  & \textbf{3.87 $\pm$1.40}  & 5.35      & 5.00     & 5.20  & 5.02           & 4.93       & 4.80          \\ \cline{2-10} 
                         & MIS (95\% CI) & -     & 24.35                    & 39.76     & 18.32    & 29.04 & \textbf{18.26} & 27.61      & 32.21         \\ \cline{2-10} 
                         & Interval      & -     & 6.14                     & 5.80      & 12.42    & 8.38  & 12.46          & 8.99       & 8.73          \\ \cline{2-10} 
                         & MIS (90\% CI) & -     & 21.77                    & 25.28     & 14.91    & 19.05 & \textbf{14.87} & 19.14      & 23.17         \\ \cline{2-10} 
                         & Interval      & -     & 5.17                     & 4.69      & 9.85     & 7.89  & 9.89           & 7.54       & 6.09          \\ \cline{2-10} 
                         & MIS (80\% CI) & -     & 14.80                    & 16.38     & 11.79    & 13.53 & \textbf{11.68} & 13.56      & 15.95         \\ \cline{2-10} 
                         & Interval      & -     & 4.04                     & 3.56      & 6.89     & 6.92  & 7.09           & 5.88       & 4.33          \\ \hline
\multirow{8}{*}{30 mins} & MAE           & 3.15  & 2.93 $\pm$ 1.30 & 3.19      & 2.79     & 3.10  & 3.08           & 2.94       & \textbf{2.54}        \\ \cline{2-10} 
                         & RMSE          & 6.45  & \textbf{5.34 $\pm$ 2.04} & 6.58      & 6.00     & 6.36  & 5.95           & 6.08       & 5.59          \\ \cline{2-10} 
                         & MIS (95\% CI) & -     & 31.68                    & 38.48     & 21.54    & 40.93 & 21.09          & 33.38      & 31.87         \\ \cline{2-10} 
                         & Interval      & -     & 8.48                     & 7.86      & 13.48    & 8.37  & 13.99          & 11.10      & 12.62         \\ \cline{2-10} 
                         & MIS (90\% CI) & -     & 23.24                    & 25.60     & 17.62    & 25.17 & \textbf{17.16} & 23.03      & 24.18         \\ \cline{2-10} 
                         & Interval      & -     & 7.15                     & 6.36      & 10.51    & 7.87  & 10.95          & 9.32       & 9.08          \\ \cline{2-10} 
                         & MIS (80\% CI) & -     & 16.31                    & 17.32     & 13.94    & 16.78 & \textbf{13.59} & 16.25      & 17.41         \\ \cline{2-10} 
                         & Interval      & -     & 5.57                     & 4.85      & 7.23     & 6.91  & 7.56           & 7.26       & 6.47          \\ \hline
\multirow{8}{*}{60 mins} & MAE           & 3.60  & 3.29 $\pm$ 1.58          & 3.99      & 3.19     & 3.75  & 3.65           & 3.70       & \textbf{3.00} \\ \cline{2-10} 
                         & RMSE          & 7.60  & 6.74 $\pm$ 2.62          & 7.98      & 7.05     & 7.91  & 6.98           & 7.76       & \textbf{6.41} \\ \cline{2-10} 
                         & MIS (95\% CI) & -     & 34.03                    & 38.58     & 25.74    & 60.56 & \textbf{24.33} & 43.11      & 30.35         \\ \cline{2-10} 
                         & Interval      & -     & 13.30                    & 11.65     & 14.50    & 8.38  & 15.55          & 14.46      & 18.79         \\ \cline{2-10} 
                         & MIS (90\% CI) & -     & 28.87                    & 27.29     & 21.18    & 35.23 & \textbf{19.95} & 29.68      & 24.59         \\ \cline{2-10} 
                         & Interval      & -     & 9.98                     & 9.45      & 11.06    & 7.88  & 11.99          & 12.14      & 14.45         \\ \cline{2-10} 
                         & MIS (80\% CI) & -     & 19.84                    & 19.58     & 16.71    & 22.06 & \textbf{16.08} & 20.88      & 19.20         \\ \cline{2-10} 
                         & Interval      & -     & 8.71                     & 7.28      & 7.45     & 6.91  & 7.88           & 9.46       & 10.42         \\ \hline
\end{tabular}
\caption{Performance comparison of different UQ methods }
\label{tab_comp}
\end{table*}

\begin{table}[!t]
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{T} & MAE (80\% CI) & MAE (90\% CI) & MAE (95\% CI) \\ \hline
15 mins              & 2.24 $\pm$ 1.01     & 2.28 $\pm$ 1.02    & 2.32 $\pm$ 1.03     \\ \hline
30 mins              & 2.64 $\pm$ 1.27     & 2.76 $\pm$ 1.17     & 2.83 $\pm$ 1.29    \\ \hline
60 mins              & 3.32 $\pm$ 1.73    & 3.49 $\pm$ 1.73    & 3.61 $\pm$ 1.73     \\ \hline
\end{tabular}\caption{Aleatoric Uncertainty Estimation using Simultaneous Quantile Regression}
\label{tab_sqr}
\end{table}s

==> extra.tex <==
\begin{table*}[!ht]\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
T                        & Metric        & DCRNN & Deep Ensembles           & Bootstrap & Quantile & SQ    & MIS            & MC Dropout & SG-MCMC       \\ \hline
\multirow{8}{*}{15 mins} & MAE           & 2.77  & \textbf{2.16 $\pm$ 0.91} & 2.63      & 2.43     & 2.67  & 2.63           & 2.47       & 2.32          \\ \cline{2-10} 
                         & RMSE          & 5.38  & \textbf{3.87 $\pm$1.40}  & 5.35      & 5.00     & 5.20  & 5.02           & 4.93       & 4.80          \\ \cline{2-10} 
                         & MIS (95\% CI) & -     & 24.35                    & 39.76     & 18.32    & 29.04 & \textbf{18.26} & 27.61      & 32.21         \\ \cline{2-10} 
                         & Interval      & -     & 6.14                     & 5.80      & 12.42    & 8.38  & 12.46          & 8.99       & 8.73          \\ \cline{2-10} 
                         & MIS (90\% CI) & -     & 21.77                    & 25.28     & 14.91    & 19.05 & \textbf{14.87} & 19.14      & 23.17         \\ \cline{2-10} 
                         & Interval      & -     & 5.17                     & 4.69      & 9.85     & 7.89  & 9.89           & 7.54       & 6.09          \\ \cline{2-10} 
                         & MIS (80\% CI) & -     & 14.80                    & 16.38     & 11.79    & 13.53 & \textbf{11.68} & 13.56      & 15.95         \\ \cline{2-10} 
                         & Interval      & -     & 4.04                     & 3.56      & 6.89     & 6.92  & 7.09           & 5.88       & 4.33          \\ \hline
\multirow{8}{*}{30 mins} & MAE           & 3.15  & 2.93 $\pm$ 1.30 & 3.19      & 2.79     & 3.10  & 3.08           & 2.94       & \textbf{2.54}        \\ \cline{2-10} 
                         & RMSE          & 6.45  & \textbf{5.34 $\pm$ 2.04} & 6.58      & 6.00     & 6.36  & 5.95           & 6.08       & 5.59          \\ \cline{2-10} 
                         & MIS (95\% CI) & -     & 31.68                    & 38.48     & 21.54    & 40.93 & 21.09          & 33.38      & 31.87         \\ \cline{2-10} 
                         & Interval      & -     & 8.48                     & 7.86      & 13.48    & 8.37  & 13.99          & 11.10      & 12.62         \\ \cline{2-10} 
                         & MIS (90\% CI) & -     & 23.24                    & 25.60     & 17.62    & 25.17 & \textbf{17.16} & 23.03      & 24.18         \\ \cline{2-10} 
                         & Interval      & -     & 7.15                     & 6.36      & 10.51    & 7.87  & 10.95          & 9.32       & 9.08          \\ \cline{2-10} 
                         & MIS (80\% CI) & -     & 16.31                    & 17.32     & 13.94    & 16.78 & \textbf{13.59} & 16.25      & 17.41         \\ \cline{2-10} 
                         & Interval      & -     & 5.57                     & 4.85      & 7.23     & 6.91  & 7.56           & 7.26       & 6.47          \\ \hline
\multirow{8}{*}{60 mins} & MAE           & 3.60  & 3.29 $\pm$ 1.58          & 3.99      & 3.19     & 3.75  & 3.65           & 3.70       & \textbf{3.00} \\ \cline{2-10} 
                         & RMSE          & 7.60  & 6.74 $\pm$ 2.62          & 7.98      & 7.05     & 7.91  & 6.98           & 7.76       & \textbf{6.41} \\ \cline{2-10} 
                         & MIS (95\% CI) & -     & 34.03                    & 38.58     & 25.74    & 60.56 & \textbf{24.33} & 43.11      & 30.35         \\ \cline{2-10} 
                         & Interval      & -     & 13.30                    & 11.65     & 14.50    & 8.38  & 15.55          & 14.46      & 18.79         \\ \cline{2-10} 
                         & MIS (90\% CI) & -     & 28.87                    & 27.29     & 21.18    & 35.23 & \textbf{19.95} & 29.68      & 24.59         \\ \cline{2-10} 
                         & Interval      & -     & 9.98                     & 9.45      & 11.06    & 7.88  & 11.99          & 12.14      & 14.45         \\ \cline{2-10} 
                         & MIS (80\% CI) & -     & 19.84                    & 19.58     & 16.71    & 22.06 & \textbf{16.08} & 20.88      & 19.20         \\ \cline{2-10} 
                         & Interval      & -     & 8.71                     & 7.28      & 7.45     & 6.91  & 7.88           & 9.46       & 10.42         \\ \hline
\end{tabular}
\caption{Performance comparison of different UQ methods }
\label{tab_comp}
\end{table*}

\begin{table}[!t]
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{T} & MAE (80\% CI) & MAE (90\% CI) & MAE (95\% CI) \\ \hline
15 mins              & 2.24 $\pm$ 1.01     & 2.28 $\pm$ 1.02    & 2.32 $\pm$ 1.03     \\ \hline
30 mins              & 2.64 $\pm$ 1.27     & 2.76 $\pm$ 1.17     & 2.83 $\pm$ 1.29    \\ \hline
60 mins              & 3.32 $\pm$ 1.73    & 3.49 $\pm$ 1.73    & 3.61 $\pm$ 1.73     \\ \hline
\end{tabular}\caption{Aleatoric Uncertainty Estimation using Simultaneous Quantile Regression}
\label{tab_sqr}
\end{table}s
